DeepRicci: Self-supervised Graph Structure-Feature Co-Refinement for Alleviating Over-squashing

Graph Neural Networks (GNNs) have shown great power for learning and mining on graphs, and Graph Structure Learning (GSL) plays an important role in boosting GNNs with a refined graph. In the literature, most GSL solutions either primarily focus on structure refinement with task-specific supervision (i.e., node classification), or overlook the inherent weakness of GNNs themselves (e.g., over-squashing), resulting in suboptimal performance despite sophisticated designs. In light of these limitations, we propose to study self-supervised graph structure-feature co-refinement for effectively alleviating the issue of over-squashing in typical GNNs. In this paper, we take a fundamentally different perspective of the Ricci curvature in Riemannian geometry, in which we encounter the challenges of modeling, utilizing and computing Ricci curvature. To tackle these challenges, we present a self-supervised Riemannian model, DeepRicci. Specifically, we introduce a latent Riemannian space of heterogeneous curvatures to model various Ricci curvatures, and propose a gyrovector feature mapping to utilize Ricci curvature for typical GNNs. Thereafter, we refine node features by geometric contrastive learning among different geometric views, and simultaneously refine graph structure by backward Ricci flow based on a novel formulation of differentiable Ricci curvature. Finally, extensive experiments on public datasets show the superiority of DeepRicci, and the connection between backward Ricci flow and over-squashing. Codes of our work are given in https://github.com/RiemanGraph/.

==> arXiv/abstract.tex <==
%!TEX root = ./DM271_DeepRicci.tex

\begin{abstract}
Graph Neural Networks (GNNs) have shown great power for learning and mining on graphs, 
and Graph Structure Learning (GSL) plays an important role in boosting GNNs with a refined graph. 
In the literature, most GSL solutions 
either primarily focus on structure refinement with task-specific supervision (i.e., node classification),
or overlook the inherent weakness of GNNs themselves (e.g., over-squashing), resulting in suboptimal performance despite  sophisticated designs.
In light of these limitations, 
% we propose a novel formulation for effectively alleviating the issue of over-squashing in typical GNNs by jointly refining graph structure and features through self-supervision.
we propose to study self-supervised graph structure-feature co-refinement for effectively alleviating the issue of over-squashing in typical GNNs.
%with theoretical guarantees.
\emph{In this paper, we take a fundamentally different perspective of the Ricci curvature in Riemannian geometry}, in which we encounter the challenges of modeling, utilizing and computing Ricci curvature. 
To tackle these challenges, we present a self-supervised Riemannian model, \emph{DeepRicci}.
Specifically,
we introduce a latent Riemannian space of heterogeneous curvatures to model various Ricci curvatures, 
and propose a gyrovector feature mapping to utilize Ricci curvature for typical GNNs.
Thereafter, we refine node features by geometric contrastive learning among different geometric views, and simultaneously refine graph structure by backward Ricci flow based on a novel formulation of differentiable Ricci curvature.
Finally, extensive experiments on public datasets show the superiority of  DeepRicci, and the connection between backward Ricci flow and over-squashing.
Codes of our work are given in \emph{https://github.com/RiemanGraph/}.
\end{abstract}


==> arXiv/body.tex <==
%!TEX root = ./DM271_DeepRicci.tex

\section{Introduction}

Graphs are ubiquitous structures representing objects (nodes) and complex interactions among them, such as social networks, academic networks, biological networks, etc., 
and Graph Neural Networks (GNNs) is becoming the dominant solution for learning and mining on graphs \cite{DBLP:conf/iclr/KipfW17,DBLP:conf/nips/HamiltonYL17,DBLP:journals/tnse/LiuWDY22,DBLP:journals/tnn/ChenGWWXLLWL22}.
GNNs typically rely on one basic assumption that the input graph is reliable. 
However, this assumption is usually unrealistic. The graph structure is often noisy with missing or redundant edges \cite{DBLP:conf/kdd/LiL0CFY022,DBLP:journals/tnn/ChenGMWWWDLW22}.
%Also, GNNs trend to encounter the phenomenon of over-squashing when the graph structure is not preferred \cite{DBLP:conf/cikm/SunLYFPJLY22,DBLP:conf/iclr/ToppingGC0B22}.
%when information passes through the bottleneck on the graph
Also, GNNs suffer from the side effect of message-passing paradigm  \cite{DBLP:conf/iclr/ToppingGC0B22}.
They both lead to the suboptimal performance of GNNs in the downstream tasks.
%as well as the perturbation from adversarial attacks \cite{DBLP:conf/kdd/LiL0CFY022}. 
Thus, it becomes a hot research topic to learn an optimized graph for boosting GNNs, referred to as Graph Structure Learning (GSL).

% \textbf{Problem.} On the one hand, most GSL is jointly optimized with node classification, the typical subsequent learning task. 
% That is, GSL requires node labels to optimize graph structure. 
% However, the supervision signal on the nodes is not well aligned with GSL target of learning an optimized structure among the nodes, 
% and thereby self-supervised GSL becomes the new paradigm very recently. 
% One the other hand, ...
% Thus, we pose a new problem of \emph{self-supervised graph structure-feature refinement} in this paper.

% In the literature, most GSL methods focus on refining graph structure in a supervised scenario, i.e., graph structure is jointly optimized with a specific downstream task (node classification).
% In the literature, most GSL methods jointly optimize graph structure and a specific downstream task of node classification, 
% i.e., supervisedly refining graph structure with the node labels \cite{DBLP:conf/aaai/Sun0P0FJY22,DBLP:conf/www/ZouPHYLWLY23,DBLP:conf/nips/WuZLWY22,DBLP:conf/kdd/SongZK22,DBLP:conf/www/LiuWWC0S22}.
% %inspiring 
% While achieving encouraging results, they still present several limitations.
% (1) The supervision signal is task-specific, and thereby the learnt structure usually cannot benefit other applications, e.g., node clustering.
% Also, the reliance of node labels may be questionable.
% (2) The few self-supervised methods solely focus on noisy graph structure \cite{DBLP:conf/www/LiuZZCPP22,DBLP:conf/wsdm/0002WJZ023}, but node features are often noisy as well.
% %This is troublesome 
% This is depressing since even if the structure is refined, node encodings generated by the GNN are still based on noisy node features.
% (3) Most GSL methods ignore the systematic weakness of GNNs themselves.



% On the one hand, most GSL methods need supervision from node classification for the structure refinement only 
% % On the one hand, most GSL methods jointly optimize graph structure and a specific downstream task of node classification \cite{DBLP:conf/www/ZouPHYLWLY23,DBLP:conf/nips/WuZLWY22,DBLP:conf/kdd/SongZK22,DBLP:conf/www/LiuWWC0S22, DBLP:conf/cikm/SunLYFPJLY22}.
% The supervision signal is task-specific and, consequently, the learnt structure usually cannot benefit other applications such as node clustering.
% %As a result, the learnt structure usually cannot benefit other applications, e.g., node clustering.
% It motivates the self-supervised GSL. 
% Same as the supervised counterpart, the recent self-supervised methods still mainly focus on structure refinement \cite{DBLP:conf/www/LiuZZCPP22,DBLP:conf/wsdm/0002WJZ023}. 
% % Same as the majority of the supervised methods, the recent self-supervised methods  still solely focus on the graph structure, which tends to be noisy.
% Nevertheless, node features are often noisy as well.
% This is depressing since even if the structure is refined, GNN still learns knowledge from the noisy features, and results in suboptimal performance on downstream tasks.
% Thus, it calls for feature refinement.

While achieving encouraging results, it still presents several limitations.
On the one hand, both traditional supervised GSL solutions \cite{DBLP:conf/www/ZouPHYLWLY23,DBLP:conf/nips/WuZLWY22,DBLP:conf/kdd/SongZK22,DBLP:conf/www/LiuWWC0S22, DBLP:conf/cikm/SunLYFPJLY22} and the recent self-supervised ones \cite{DBLP:conf/www/LiuZZCPP22,DBLP:conf/wsdm/0002WJZ023} primarily focus on the structure refinement, i.e., refining the graph structure which tends to be noisy.
However, node features are often noisy as well.
This is problematic, because even if the structure is refined, GNN still learns from the noisy features, leading to suboptimal performance in downstream tasks.
Therefore, there is a need for the co-refinement of both graph structure and node feature to achieve better performance.
On the other hand, most GSL methods, including the recent \cite{DBLP:conf/www/LiuZZCPP22,DBLP:conf/wsdm/0002WJZ023}, overlook the inherent weakness of the message-passing within typical GNNs \cite{DBLP:conf/iclr/KipfW17,DBLP:conf/nips/HamiltonYL17,DBLP:conf/iclr/VelickovicCCRLB18}.
% For instance, the valuable information on the nodes is squashed when passing through the bottlenecks on the graph, especially for the information from the long-distant nodes  
When a large volume of messages passes through a narrow path in the graph, the useful information tends to be distorted and squashed \cite{DBLP:conf/cikm/SunLYFPJLY22}.
This phenomenon, known as ``\emph{over-squashing}'', usually limits the expressive power of GNNs.
Besides, the supervised GSL \cite{DBLP:conf/cikm/SunLYFPJLY22} that relies on the supervision for node classification usually cannot benefit other applications, e.g., node clustering. On the contrary, self-supervised GSL is preferable for learning  generic knowledge.
In light of these limitations, 
we propose to study self-supervised graph structure-feature co-refinement for effectively alleviating the phenomenon of over-squashing in typical GNNs.
% To the best of our knowledge, the few GSL methods that address the over-squashing, such as \cite{DBLP:conf/cikm/SunLYFPJLY22}, are supervised by the node labels.
% In light of these limitations, we put forward a novel problem of \emph{self-supervised graph structure-feature refinement, jointly relieving the over-squashing of typical GNNs}.
% we propose a novel formulation for effectively alleviating the issue of over-squashing in typical GNNs by jointly refining the graph structure and features through self-supervision.
% \textbf{Challenges.} We notice that model interpretability in GSL is largely under-explored. For example, it is unclear why the learnt graph is able to relieve \emph{over-squashing}, a significant phenomenon limiting the expressive power of GNNs.
%To date,  in general lacks a theory, especially for learning a optimized structure to relieve form the phenomenon of \emph{over-squashing}. 
%Recently, Ricci curvature, describing the high-order connectivity on graph structure,  ... 

% In Riemannian geometry, a each edge in the graph is attached to a Ricci curvature describing the high-order connectivity between the two endpoints.
% each pair of nodes in the graph is associated with a Ricci curvature describing the high-order connectivity between them \cite{RicciCurvatureOfGraph}.
%Recent studies show that, the phenomenon of over-squashing is inherently connected to the notion of Ricci curvature  \cite{DBLP:conf/iclr/ToppingGC0B22,DBLP:conf/www/Liu0P00C023}.
In Riemannian geometry, Ricci curvatures on a graph describe the high-order connectivity between node pairs \cite{RicciCurvatureOfGraph}, shedding lights on the structure learning.
%It is not until very recently that 
Very recently, Ricci curvature is also connected to the phenomenon of over-squashing \cite{DBLP:conf/iclr/ToppingGC0B22,DBLP:conf/www/Liu0P00C023},
\textbf{motivating us to address GSL from a fundamentally different perspective of Riemannian geometry.}
However, we are facing the following challenges: 

\emph{Challenge 1: How to model Ricci curvature in the representation space?} 
Most representation spaces typically assume  a single uniform curvature radius, such as Euclidean, hyperbolic, spherical spaces and, more recently, quotient/ultrahyperbolic manifolds \cite{DBLP:conf/nips/XiongZPP0S22,DBLP:conf/nips/Law21}. 
However, Ricci curvatures indeed imply a representation space that exhibits  diverse curvatures over the edges/nodes.
%it lacks a promising space allowing different regions have different curvatures, so as to model Ricci curvature for GSL. 
In short, there is a lack of a promising space that enables different regions to have distinct curvatures, which is necessary for modeling Ricci curvature for GSL.

\emph{Challenge 2: How to utilize Ricci curvature for typical GNNs?} 
As mentioned above, Ricci curvature is built in Riemannian geometry, but the vast majority of GNNs \cite{DBLP:conf/iclr/KipfW17,DBLP:conf/nips/HamiltonYL17,DBLP:conf/iclr/VelickovicCCRLB18} work with the Euclidean space.
%The mathematicians show that, 
There is no isomorphism connecting the two types of spaces due to the inherent distinction in geometry \cite{RieGeo}. 
In other words, even if an appropriate representation space is designed, 
the challenge of bridging it to the Euclidean space for typical GNNs remains unresolved.
%how to bridge it to the Euclidean one for typical GNNs still remains open.
% Ricci curvature cannot be directly applied to Euclidean GNNs, owing to the inherent distinction in geometry. 
% More importantly, there exists no isomorphism connecting the two kinds of spaces, making this problem tougher. 

\emph{Challenge 3: How to compute Ricci curvature in a differentiable way?}
Ricci curvature is well defined in discrete problems, such as finding an optimal transport \cite{Olli2010Survey} or enumerating triangles \cite{DBLP:conf/iclr/ToppingGC0B22}.
However, solving discrete problem blocks the gradient backpropagation, preventing the joint learning of graph structure and curvature.
This poses the fundamental challenge to a learning model, and also explains why aforementioned methods \cite{DBLP:conf/iclr/ToppingGC0B22,DBLP:conf/www/Liu0P00C023} cannot be used for GSL.


\textbf{Present Work.}
To bridge the technical gaps, we propose a self-supervised GSL model, \textbf{DeepRicci}.
 %, \textbf{a self-supervised model for the joint structure-feature refinement}.
The novelty lies in that we introduce a \emph{latent Riemannian space}
%\footnote{We utilize the terminologies of ``space'' and ``manifold'' interchangeably throughout this paper.} 
in which we simultaneously refine graph structure and node features, alleviating the over-squashing on the graph.
To address challenge one, 
we construct the latent Riemannian space using a rotational product,  
%in which node feature is concatenated with learnable parameters for refinement.
and demonstrate that our design enables different nodes having different curvature, thereby facilitating the modeling of the various Ricci curvatures on the graph.
To address challenge two, 
we propose a gyrovector  feature mapping to bridge between the Riemannian manifold and Euclidean space with an isometry-invariant kernel.
To address challenge three, 
we introduce a differentiable formulation of Ricci curvature based on Olliver's definition \cite{Olli2010Survey}, replacing the discrete counterpart.
%we formulate a differentiable Ricci curvature following the Olliver's definition to replace the discrete one.
In reminiscent of the famous Ricci flow, \emph{graph structure is refined} in the backward Ricci flow with the differentiable curvature.
\emph{Node feature is simultaneously refined} in the contrasting learning among different geometric views induced from the product factors.
%    
%Last but not least,  
Furthermore, we prove that the graph learnt by DeepRicci 
\emph{alleviates the over-squashing by increasing the Cheeger’s constant on the graph}.
%minimum positive Ricci curvature


Overall, main contributions are summarized as follows.
\begin{itemize}
\item \emph{Problem.} In this paper, we propose a new problem of self-supervised graph structure-feature co-refinement, alleviating the over-squashing phenomenon in GNNs.
% and providing 
\item \emph{Methodology.} We take a fundamentally different perspective of Riemannian geometry, and propose the first Riemannian graph learning model (DeepRicci), to our best  knowledge. We introduce a latent Riemannian space, gyrovector  feature mapping and differential Ricci curvature with several theoretical guarantees. 
\item \emph{Experiment.} Extensive experiments on 4 public datasets show the superiority of DeepRicci.
 %that  DeepRicci outperforms the state-of-the-art methods. 
 Furthermore, we empirically show the connection between Ricci flow and the over-squashing.
\end{itemize}


\begin{figure*}
\centering
    \includegraphics[width=0.95\linewidth]{illu6}
            \vspace{-0.05in}
     \caption{Overall architecture of \textbf{DeepRicci}. We introduce a latent Riemannian space, constructed by rotational product (\textbf{Sec. \ref{TheSpace},B}), in which we jointly refine structure with backward Ricci flow (\textbf{Sec. \ref{DiffRiccCurv},D}) and refine feature by geometric contrastive learning (\textbf{Sec. \ref{SecOfFeatureRefine}}). A few linkages are added in the output graph  to alleviate the ``\emph{bottleneck}'' of the input graph (\textbf{Sec. \ref{theory}}).}
    \label{illu}
        \vspace{-0.2in}
\end{figure*}

       \vspace{-0.03in}
\section{Preliminaries}
        \vspace{-0.03in}
We first introduce the fundamental notion of manifold and curvature in Riemannian geometry.
% including the notions of  manifold and curvature. 
Then, we put forward a new problem of \emph{self-supervised graph structure-feature co-refinement}, and point out its challenges.
% a more practical yet challenging problem we focused on in this paper.
        \vspace{-0.05in}
\subsection{Riemannian Geometry}
        \vspace{-0.03in}
\subsubsection{Manifold}
A smooth manifold $\mathcal M^d$ is said to be a Riemannian manifold if it is endowed with a Riemannian metric $g$, where $d$ is the dimensionality.
Each point $x \in \mathcal M$ is associated with a tangent space $\mathcal T_x\mathcal M^d \in \mathbb R^d$ around $x$ where the metric $g$ is defined, controlling the shape of the manifold.
%The Riemannian metric is a collection of inner product 
Mapping between the tangent space and the manifold is done via exponential and logarithmic maps. 
In particular, the logarithmic map at $x$ does $log_x(\cdot): \mathcal M \to \mathcal T_x\mathcal M$, while the exponential map acts inversely.
%The \emph{exponential map} projects from the tangent space onto the manifold, and the \emph{logarithmic map} does inversely \citep{2013manifold}.
%The notion of curvature
%a curve deviates from being a straight line, or 
\subsubsection{Curvature}
The curvature describes the extent how a surface deviates from being a plane. 
For $\boldsymbol x \in \mathcal M$, the sectional curvature $\kappa_x$ is defined on its tangent space $\mathcal T_x \mathcal M$.
A unit tangent vector $\boldsymbol v \in \mathcal T_x \mathcal M$ is associated with a Ricci curvature defined by averaging the sectional curvatures of planes containing $\boldsymbol v$, 
and the Ricci curvature controls the overlap of two balls w.r.t. the radii and the distance between their centers.

%Given a tangent vector , the Ricci curvature is defined averaging 

% As shown in 
% Most of graph structure learning works seek to solely optimize the adjacency matrix $\boldsymbol A$ for downstream tasks.
% %As node features are not reliable as well, we pose a problem of more practical yet challenging setting as follows.
% However, neither graph structure nor node features are reliable in practice, and thereby we pose a  new problem of more challenging setting as follows.
%we consider a more practical yet challenging setting that both graph structure and node features are noisy.

       \vspace{-0.03in}
\subsection{Problem Formulation}
       \vspace{-0.03in}
A graph $G(\boldsymbol A, \boldsymbol X)$ is defined on a node set $\mathcal V=\{v_1, \cdots, v_N\}$,
where $\boldsymbol A \in \mathbb R^{|\mathcal V|\times |\mathcal V|}$ is the binary adjacency matrix describing the graph structure. 
We have $[\boldsymbol A]_{ij}=1$ iff the nodes $v_i$ and $v_j$ are linked, otherwise, $[\boldsymbol A]_{ij}=0$.
Each node is attached with a feature $\boldsymbol x_i \in \mathbb R^F$, summarized in $\boldsymbol X \in \mathbb R^{|\mathcal V|\times F}$.
GNNs typically conduct message-passing over the graph structure with node features as the network input \cite{DBLP:conf/iclr/KipfW17,DBLP:conf/nips/HamiltonYL17,DBLP:conf/iclr/VelickovicCCRLB18}. 
%The bottlenecks on the graph structure tend to result in the over-squashing, and thus limit the power of GNNs.
GSL aims at boosting the performance of GNNs with an optimized graph. 
In this paper, we argue that \emph{not only graph structure but also node feature} affect the performance of GNN, given that both of them tend to be noisy in reality.
Thus, we explore a practical and challenging problem.
\newtheorem*{def1}{The Problem of Self-supervised Graph Structure-Feature Co-Refinement} 
\begin{def1}
Given a graph $G(\boldsymbol A, \boldsymbol X)$ with noisy structure $\boldsymbol A$ as well as noisy features $\boldsymbol X$,  
the target of self-supervised structure-feature co-refinement is to learn an optimized graph $G^\star(\boldsymbol A^\star, \boldsymbol X^\star)$ without supervision signals. 
The refined adjacency matrix $\boldsymbol A^\star \in [0, 1]^{N \times N}$ 
better encodes the underlying dependency between nodes with a latent Riemannian manifold $\mathcal M$, 
boosts the performance of downstream tasks  together with the refined node feature $\boldsymbol X^\star$, 
and  alleviates the over-squashing in the message-passing  of typical GNNs.
\end{def1}

In short, we are interested in jointly refining graph structure and node features, and alleviating over-squashing in absence of label information on the nodes or any downstream tasks.
%\textbf{Essentially different from existing solutions, we rethink GSL from a fundamentally different perspective of Riemannian geometry.} 
\textbf{Fundamentally different from existing solutions, we approach GSL from a fresh perspective rooted in Riemannian geometry.}
Though Riemannian geometry provides elegant theory to study graph structures, e.g., Ricci curvature, we are still facing tremendous challenges. 

       \vspace{-0.03in}
\subsection{Challenges}
       \vspace{-0.03in}
\subsubsection{Homogeneous vs. Heterogeneous Space}
In Riemannian geometry, a smooth manifold is a \emph{homogeneous (curvature) space} if the sectional curvature is equal everywhere in the manifold.
A homogeneous space is characterized by the sectional curvature denoted as $\kappa$, since its value is regardless of $\boldsymbol x$. 
Correspondingly, the curvature radius is given as $\frac{1}{|\kappa|}$.
In particular, a $d-$dimensional homogeneous space is hyperbolic $\mathbb H^d_\kappa$ when $\kappa<0$. It is hyperspherical $\mathbb S^d_\kappa$ when  $\kappa>0$. 
Euclidean space $\mathbb R^d$ is a special case with $\kappa=0$. 
In the literature of graph data mining, most of the representation spaces are homogeneous  \cite{DBLP:conf/nips/ChamiYRL19,DBLP:conf/nips/LiuNK19,DBLP:conf/www/ZhangWSLS21,DBLP:conf/cvpr/DaiWGJ21,DBLP:conf/acl/ChenHLZLLSZ22}, including the recent studies \cite{DBLP:conf/nips/XiongZPP0S22,DBLP:conf/nips/Law21}.
They present a singe curvature radius $\kappa$, and thus lack the ability to model the various curvatures on the graph, posing \textbf{Challenge 1}.
Indeed, it calls for a \emph{heterogeneous (curvature) space} in which different points have different curvatures.
Furthermore, we are interested in boosting the performance of typical GNNs in the Euclidean space \cite{DBLP:conf/iclr/KipfW17,DBLP:conf/nips/HamiltonYL17,DBLP:conf/iclr/VelickovicCCRLB18}.
However, it still unclear how to bridge between a heterogeneous space and Euclidean space, and thus poses \textbf{Challenge 2}.

\subsubsection{Ricci Curvature}
The overlap of two balls is inherently connected to the cost of transportation moving one ball to the other, yielding the Ollivier definition of Ricci curvature \cite{Olli2010Survey}.
In a graph, 
given the mass distribution $m_u^\alpha(v)$  node $u \in \mathcal{V}$, 
\vspace{-0.03in}
\begin{equation}
    m_u^\alpha(v)=
    \begin{cases}
    \alpha, & v = u,\\
    (1 - \alpha)\frac{1}{|\mathcal N(u)|},& v \in \mathcal N(u), \\
    0, & Otherwise,
    \end{cases} \label{pmf}
    \vspace{-0.03in}
\end{equation}
where $\mathcal N(u)$ is the set of nodes linking to  $u$.
The Ollivier's Ricci curvature of a node pair $(i, j)$ is defined as follows:
\vspace{-0.03in}
\begin{equation}
    {Ric}^{\alpha}(i, j) = 1 - \frac{W(m_i^\alpha, m_j^\alpha)}{d(i, j)},
    \label{ORC}
    \vspace{-0.03in}
\end{equation}
where $W(m_i^\alpha, m_j^\alpha)$ is the Wasserstein distance \cite{DBLP:conf/nips/GulrajaniAADC17} between the probability (mass) distributions on nodes $i$ and $j$, and $d(i, j)$ is the distance defined on the graph.
The other popular variant is the Forman's Ricci curvature \cite{DBLP:conf/iclr/ToppingGC0B22}, whose definition involves triangle enumeration on the graph.
In other words, both definitions measure Ricci curvature with a discrete optimization problem, and thus blocks the gradient backpropagation for graph learning, posing \textbf{Challenge 3}.

%shortest path on graph from node $u$ to node $v$.

% \textbf{Notations.} Bold uppercase letter and bold lowercase letter denote matrix and vector, respectively. $\langle \cdot, \cdot \rangle$ and $|\cdot|$ denote the standard inner product and usual $L2$ norm.




\section{Our Approach: DeepRicci}

We present a self-supervised Riemannian model for graph structure-feature co-refinement, named as \textbf{DeepRicci}.
In a nutshell, we introduce a \emph{latent Riemannian space} with \emph{gyrovector  feature mapping},
in which we refine node features by the contrastive learning among different geometric views, 
and simultaneously refine graph structure with \emph{backward Ricci flow} based on a novel formulation of \emph{differentiable Ricci curvature}, alleviating the over-squashing on the graph.

The overall architecture of DeepRicci is sketched in Fig. \ref{illu}.

\noindent Before detailing the co-refinement mechanism, we first introduce the manifold  in which we build our model.

\vspace{-0.03in}
\subsection{Rotational Product Construction}\label{TheSpace}
\vspace{-0.03in}

We introduce a \emph{Latent Riemannian Space} $\mathcal M$, which is a heterogeneous manifold constructed by a carefully designed rotational  product,  addressing Challenge 1.
% construction to model the fine-granularity Ricci curvatures.

Specifically, we design the \emph{rotational  product} as follows,
\begin{equation}
\mathcal M = \mathcal P \otimes \mathcal F, \  \mathcal P=\otimes_{m=1}^{M-1}{\mathbb G}_{\kappa_m}^{d_m}, \ M \ge 2.
\end{equation}
$\mathcal M$ is the product of $M$ factor space, and the $M^{th}$ factor is the \emph{rotational factor}. $\otimes$ denotes the Cartesian product of manifolds. 
In the Cartesian product, a point in the product space $\boldsymbol x \in \mathcal M$ is expressed as 
\vspace{-0.03in}
\begin{equation}
\boldsymbol x=\operatorname{Concat}(\boldsymbol x^{\kappa_1}, \cdots, \boldsymbol x^{\kappa_m}, \cdots, \boldsymbol x^{\kappa_M}), \ \  \boldsymbol x^{\kappa_m} \in \mathbb G^{d_m}_{\kappa_m},
\vspace{-0.03in}
\end{equation}
where $\operatorname{Concat}(\cdot)$ denotes the operation of concatenation.
$\boldsymbol x^{\kappa_m} $ is the component of $\boldsymbol x$ in the $m^{th}$ factor.
The dimension of the product $\mathcal P$ is the sum of dimension of each factor $d=\sum\nolimits_{m=1}^{M-1} d_m$.
The distance between $\boldsymbol x$ and  $\boldsymbol y$ is given in  $d^2_{\mathcal P}(\boldsymbol x, \boldsymbol y)=\sum\nolimits_{m=1}^{M-1} d^2_{\kappa_m}(\boldsymbol x^{\kappa_m}, \boldsymbol y^{\kappa_m})$.
In the designed product, we utilize the \textbf{$\boldsymbol \kappa$-stereographic model} for each factor, \emph{unifying the vector operations of the aforementioned three types of spaces with gyrovector formalism.} 
%\citep{ungar2008gyrovector}.  (Notations: Bold lowercase $\boldsymbol{x}$ and bold uppercase $\boldsymbol{X}$ denote the vector and matrix, respectively.)
Its $d$-dimensional model is a smooth manifold 
$\mathbb G^{d}_{\kappa}=\left\{\boldsymbol{x} \in \mathbb{R}^{d} \mid-\kappa |\boldsymbol{x}|^{2}<1\right\}$,
whose distance function is given as 
\begin{equation}
d(\boldsymbol x, \boldsymbol y)=\frac{2}{\sqrt{|\kappa|}}\tan^{-1}_\kappa\left(\sqrt{|\kappa|} |-\boldsymbol x \oplus_\kappa \boldsymbol y|\right),
\end{equation}
where $\oplus_\kappa$ is the gyrovector addition and $\tan^{-1}_\kappa$ is the curvature trigonometry \cite{DBLP:conf/icml/BachmannBG20}.
$\kappa$-stereographic model shifts to a hypersphere model of hyperspherical space with $\kappa > 0$, 
and to a Poincar{\'{e}} ball model of hyperbolic space with $\kappa<0$. 
In particular, the rotational factor is a upper hypersphere $\mathcal F=\bar{\mathbb G}_{+}^{d_M}$, where ${}_+$ denotes the positive curvatures.

% equipped with a Riemannian metric 
% $g_{\boldsymbol{x}}^{\kappa}=\left(\lambda_{\boldsymbol{x}}^{\kappa}\right)^{2} \boldsymbol{I}$, where $\kappa \in \mathbb{R}$ 
% is the sectional curvature and 
% $\lambda_{\boldsymbol{x}}^{\kappa}=2\left(1+\kappa\|\boldsymbol{x}\|_2^{2}\right)^{-1}$ 
% is the conformal factor defined on the point $\boldsymbol{x}$. 

%Euclidean space is the special case with $\kappa =0$. 

\newtheorem*{pro1}{Proposition 1 (Heterogeneous Manifold)} 
\begin{pro1}
The product of $\mathcal M = \mathcal P \otimes  \mathcal F$ is a heterogeneous manifold, where $\mathcal F=\bar{\mathbb G}_{+}^{d_M}$ is the upper hypersphere providing curvature heterogeneity.
\end{pro1}

\begin{proof}
We sketch the proof with the key equations and omit math details owing to the limit of space.
\emph{$\mathcal M$ is heterogeneous iff the curvature $\kappa_{\boldsymbol x}$ is a function w.r.t. the location of $\boldsymbol x \in \mathcal M$}.
In the polar coordinates of $\bar{\mathbb G}_{+}^{d_M}$, Riemannian metric of rotational symmetry is $g_\rho = dr^2 + \rho^2(r)g_{\mathbb S^{d-1}}$ with some odd $\rho$ satisfying $\partial_r \rho(0)=1$. $r$ is the coordinate of the distance from the origin  (singular orbit) in gyrovector formalism.
The sectional curvature of $\bar{\mathbb G}_{+}^{d_M}$ is given by the function
\vspace{-0.05in}
\begin{equation}
\kappa_{\operatorname{rot}}=d_M \left(-2\frac{\partial^2_{rr}\rho}{\rho} + \left(d_M-1\right)\frac{1-(\partial^2_{r}\rho)^2}{\rho^2} \right), 
\vspace{-0.05in}
\end{equation}
according to \cite{RieGeo}(Chapter 3).
In the rotational product, the sectional curvature is expressed as 
\vspace{-0.05in}
\begin{equation}
\kappa_x=\kappa_{\mathcal P} + \kappa_{\operatorname{rot}}(r).
\vspace{-0.05in}
\end{equation}
The first term is derived as  a constant \cite{DBLP:journals/corr/abs-2202-01185}, and the second varies w.r.t. the location of $\boldsymbol x$, completing the proof.
\end{proof}

%\cite{DBLP:conf/iclr/GuSGR19}
\noindent Given the polar coordinates of $\bar{\mathbb G}_{+}^{d_M}$, only $r-$coordinate contributes to curvature and distance $d_{\mathcal F}(\boldsymbol x, \boldsymbol y)=r_{\boldsymbol x}-r_{\boldsymbol y}$. 
For simplicity, we utilize the node feature $\boldsymbol x^{\operatorname{raw}}$ for $r-$coordinate, thus inducing $r=|\boldsymbol x|$ with  $d_{\mathcal F}(\boldsymbol x, \boldsymbol y)=|\boldsymbol x|-|\boldsymbol y|$.
%In practice, we set  $d_r=2$, $r=|\boldsymbol x|$, and use node feature $\boldsymbol x$ for the $r$ coordinate in $\bar{\mathbb G}_{+}^d$.
%We have $\boldsymbol z=\operatorname{Concate}(\boldsymbol z^{\mathcal P}, |\boldsymbol x|)$,
\emph{It yields an equivalent product of $\mathcal M=\mathcal P \times \mathcal F$, where $\mathcal F \in \mathbb R^F$ is the rotational factor of Euclidean features, and $\mathcal P$ is the homogeneous product of hyperspherical or hyperbolic manifolds}. 

% We have $\boldsymbol z=\operatorname{Concate}(\boldsymbol z^{\mathcal P}, |\boldsymbol x|)$,
% \emph{yielding an equivalent $\mathcal M=\mathcal P \times \mathbb R^F$ and $\mathcal P$ is the product of hyperspherical or hyperbolic manifolds}. 
%with distance $d^2(\boldsymbol x, \boldsymbol y)=d^2_{\mathcal P}(\boldsymbol x, \boldsymbol y)+|\boldsymbol x- \boldsymbol y|^2$.

\noindent \textbf{Remarks.} It is noteworthy that the product construction itself \cite{DBLP:conf/iclr/GuSGR19,DBLP:conf/icml/BachmannBG20} cannot induce a manifold of heterogeneous curvatures. 
For instance, neither $\mathbb G^{d_1}_{-1} \times \mathbb G^{d_2}_{-2}$ (product of two hyperbolic manifolds) nor $\mathbb G^{d_1}_{-1} \times \mathbb G^{d_2}_{+1}$ (product of a hyperbolic manifold and hyperspherical one) will result in a constant curvature, as shown in the \emph{Proof}.
In other words, the product space without a rotational factor is still homogeneous.

\subsection{Gyrovector Feature Mapping}\label{LMap}

In this subsection, we build a bridge between Riemannian manifold and Euclidean space, addressing Challenge 2.
To this end, we propose a gyrovector  feature mapping $\phi^\kappa: \mathbb G_\kappa^{n} \to \mathbb R^{m}$, where $\mathbb G_\kappa^{n}$ is the Riemannian manifold of gyrovector formalism, and dimensions $n$ and $m$ can be different.
% to activate the multiple geometric views of the graph.

There is no isomorphism connecting the two types of spaces \cite{RieGeo}. 
Instead, we resolve this challenge with the aid of a kernel.
In the Euclidean space, for any isometry-invariant kernel, the eigenfunctions based on the Laplace operator construct (random) \emph{Fourier feature mapping} (the famous result of Bochner’s Theorem \cite{DBLP:conf/nips/RahimiR07}).
A popular parameterization for eigenfunctions are the \textbf{plane waves} $z_{\omega, b}(\boldsymbol x)=\sqrt{2}\cos(\langle \omega, \boldsymbol x\rangle +b)$, 
yielding a real-valued mapping with an invariant kernel $\mathbb E_{\omega, b}[z_{\omega, b}(\boldsymbol x)z_{\omega, b}(\boldsymbol y)]=k(\boldsymbol x-\boldsymbol y)$,
where $\omega$ and $b$ are uniformly sampled from a unit ball and $[0, 2\pi]$, respectively.

%The Laplace-Beltrami operator

We generalize the aforementioned Fourier feature mapping to any Riemannian manifold.
% with gyrovector formalism.
%In our gyrovector  feature mapping, the \textbf{generalized  waves} is formulated as 
The generalized feature mapping is constructed with \textbf{gyrovector waves}. For any  $\boldsymbol x^\kappa \in \mathbb G_\kappa^{n}$ of $\kappa-$stereographic model, the gyrovector wave is derived as
\vspace{-0.05in}
\begin{equation}
\operatorname{GF}^\kappa_{\lambda,b, \boldsymbol \omega}(\boldsymbol x^\kappa)=\exp\left(\frac{n-1}{2}\langle \boldsymbol \omega, \boldsymbol x^\kappa \rangle_\kappa\right)\cos\left( \lambda \langle \boldsymbol \omega, \boldsymbol x^\kappa \rangle_\kappa +b \right),
\label{gyroWave}
\end{equation}
%where $d_1$ is the dimension of Riemannian manifold $\mathbb G_\kappa^{d_1}$. 
where 
$
\langle \boldsymbol \omega, \boldsymbol x^\kappa \rangle_\kappa=\frac{1}{\sqrt{|\kappa|}} \tan^{-1}_\kappa\left(\sqrt{|\kappa|}\frac{|\boldsymbol x^\kappa|^2-\langle\boldsymbol \omega, \boldsymbol x^\kappa \rangle}{1+\langle\boldsymbol \omega, \boldsymbol x^\kappa \rangle} \right)
$
is indeed the signed distance.
We draw $m$ independent samples of  $\omega$, $b$  and $\lambda$ uniformly from the unit ball, $[0, 2\pi]$ and a distribution $\rho$,  respectively.
%Note that, $\omega$ is uniformly samples on the unit ball, $\lambda$ is proportional to a distribution $\rho$ and $b$ uniformly on $[0, 2\pi]$.
Gyrovector feature mapping is then given as  
\begin{equation}
\phi^\kappa(\boldsymbol x^\kappa)=\frac{1}{\sqrt{m}}\left[\operatorname{GF}^\kappa_{\lambda_1,b_1, \boldsymbol \omega_1}(\boldsymbol x^\kappa), \cdots,\operatorname{GF}^\kappa_{\lambda_m,b_m, \boldsymbol \omega_m}(\boldsymbol x^\kappa) \right],
\end{equation}
yielding the Euclidean $\phi^\kappa(\boldsymbol x^\kappa) \in \mathbb R^{m}$.


% \begin{equation}
% \begin{aligned}
% k_\lambda(g\circ \boldsymbol x, \boldsymbol o)
% & =  \frac{1}{2}\mathbb E_{\boldsymbol \omega}\left[\zeta_{\lambda,\boldsymbol \omega}(g\circ \boldsymbol x) ^*\zeta_{\lambda,\boldsymbol \omega}(\boldsymbol o) \right]\\
% &=  \frac{1}{2}\mathbb E_{\boldsymbol \omega}\left[\zeta_{\lambda,\boldsymbol \omega}(g\circ \boldsymbol x) ^*\right],\\
% & =\frac{1}{2}\mathbb E_{  \hat{\boldsymbol \omega}  }\left[\exp\left(  n_\lambda^-  \langle \boldsymbol x, \hat{\boldsymbol \omega} \rangle_\kappa+n_\lambda^+\langle \boldsymbol y, \hat{\boldsymbol \omega} \rangle_\kappa\right)\right],
% \end{aligned}
% \end{equation}

\newtheorem*{pro2}{Proposition 2 (Isometry Invariant)} 
\begin{pro2}
The induced kernel $k(\boldsymbol x^\kappa, \boldsymbol y^\kappa)=\mathbb E\left[ \operatorname{GF}^\kappa_{\lambda,b, \boldsymbol \omega}(\boldsymbol x^\kappa) \operatorname{GF}^\kappa_{\lambda,b, \boldsymbol \omega}(\boldsymbol y^\kappa)\right]$ from the gyrovector  feature mapping is isometry invariant and real.
\end{pro2}
\begin{mymath}
\begin{proof}
According to \cite{MR1790156}, the geometric identity for any isometry $g$ is given as
$
\langle g\circ \boldsymbol x^\kappa, g\circ \boldsymbol \omega \rangle=\langle  \boldsymbol x^\kappa, \boldsymbol \omega \rangle + \langle  g\circ \boldsymbol o, g\circ \boldsymbol \omega \rangle
$,
and thereby
$
\langle g^{-1}\circ \boldsymbol o, \boldsymbol \omega \rangle =- \langle  g\circ \boldsymbol o, g\circ \boldsymbol \omega \rangle
$.
By definition, 
\vspace{-0.05in}
\begin{equation}
k_\lambda(\boldsymbol x^\kappa, \boldsymbol y^\kappa)=\frac{1}{2}\mathbb E_{\boldsymbol \omega}\left[\exp\left(  n_\lambda^-  \langle \boldsymbol x^\kappa, \boldsymbol \omega \rangle_\kappa+n_\lambda^+\langle \boldsymbol y^\kappa, \boldsymbol \omega \rangle_\kappa\right)\right],
\end{equation}
where $n_\lambda^-=\frac{n-1}{2}-i\lambda$ and $n_\lambda^+=\frac{n-1}{2}+i\lambda$.
With $g\circ \boldsymbol y=\boldsymbol o$, 
\begin{equation}
\begin{aligned}
k_\lambda(g\circ \boldsymbol x^\kappa, \boldsymbol o)
& =  \frac{1}{2}\mathbb E_{\boldsymbol \omega}\left[\zeta_{\lambda,\boldsymbol \omega}(g\circ \boldsymbol x^\kappa) ^*\zeta_{\lambda,\boldsymbol \omega}(\boldsymbol o) \right]\\
& =\frac{1}{2}\mathbb E_{  \hat{\boldsymbol \omega}  }\left[\exp\left(  n_\lambda^-  \langle \boldsymbol x^\kappa, \hat{\boldsymbol \omega} \rangle_\kappa+n_\lambda^+\langle \boldsymbol y^\kappa, \hat{\boldsymbol \omega} \rangle_\kappa\right)\right],
\end{aligned}
\end{equation}
using $\hat{\boldsymbol \omega}=g^{-1} \circ \boldsymbol \omega$ as a change of variable,
where $\zeta_{\lambda,\boldsymbol \omega}(\boldsymbol z)$
$=\exp(n_\lambda^+ \langle \boldsymbol \omega, \boldsymbol z\rangle_\kappa)$ is the eigenfunction.
We have the equality
$k_\lambda(\boldsymbol x^\kappa, \boldsymbol y^\kappa)=k_\lambda(g\circ \boldsymbol x^\kappa, \boldsymbol o)$. 
For any $k_\lambda(\boldsymbol z, \boldsymbol o)$, it is derived as
\begin{equation}
k_\lambda(\boldsymbol z, \boldsymbol o)=\frac{1}{2}F_1\left(n_\lambda^+,n_\lambda^-;\frac{n}{2};\frac{1-\cos_\kappa(d_\kappa(\boldsymbol z, \boldsymbol o))}{2}\right),
\end{equation}
where $F$ is the hypergeometric function defined by power series \cite{Yu2022RandomLF}.
\emph{It claims that $k_\lambda(\boldsymbol x^\kappa, \boldsymbol y^\kappa)$ is distance-invariant depending on $d_\kappa(\boldsymbol z, \boldsymbol o)$, and thus isometry-invariant for any $\lambda$}.
Given a distribution $\rho$ over $\lambda$, the resulting kernel is 
\begin{equation}
\resizebox{1\hsize}{!}{$
k(\boldsymbol x^\kappa, \boldsymbol y^\kappa)=\frac{1}{2}\int_{-\infty}^{\infty} F_1\left(n_\lambda^+,n_\lambda^-;\frac{n}{2};\frac{1-\cos_\kappa(d_\kappa(\boldsymbol x^\kappa, \boldsymbol y^\kappa))}{2}\right)\rho(\lambda)d\lambda.
$}
\end{equation}
The kernel is shown to be \emph{real} with Legendre function.
\end{proof}
\end{mymath}

\noindent \textbf{Remarks.} Though the logarithmic map arrives at the tangent space $\mathcal T_x\mathcal M^d \in \mathbb R^d$, it is complicated and numerical unstable \cite{DBLP:conf/cvpr/DaiWGJ21}. 
No closed-form conclusions can be drawn without privileging of the origin (i.e., using the origin as the reference point for any point on the manifold) \cite{DBLP:conf/acl/ChenHLZLLSZ22}.
In contrast, our mapping is coupled with a isometry-invariant kernel, and we will show its empirical superiority in Ablation Study.
\cite{Yu2022RandomLF} constructs isometry-invariant mapping for hyperbolic space, but ours is suitable for both hyperbolic and hyperspherical space.

\vspace{-0.05in}
\subsection{Differentiable Ricci Curvature}\label{DiffRiccCurv}

The optimal transport problem nested in Ricci curvature blocks gradient backpropagation in graph learning (Challenge 3).
To bridge this gap, we formulate a novel differentiable Ricci curvature following the Ollivier's definition.

We first define a Laplacian matrix $\boldsymbol L^\alpha$ for structure $\boldsymbol A$ as
\vspace{-0.05in}
\begin{equation}
[\boldsymbol L^\alpha]_{ij}=
\begin{cases}
\alpha, & i=j,\\
(1-\alpha)\frac{1}{\boldsymbol D_{ii}}, & [\boldsymbol A]_{ij}=1, \\
0, & Otherwise,
\end{cases} \label{alphaLaplacian}
\vspace{-0.07in}
\end{equation}
whose matrix form is given as $\boldsymbol L^\alpha= \alpha \boldsymbol I + (1-\alpha) \boldsymbol D^{-1} \boldsymbol A$, where $\boldsymbol D$ is the diagonal degree matrix.
Then, we derive the following  Ricci matrix $\boldsymbol R^\alpha(\boldsymbol A, \boldsymbol X)$, whose $(i,j)-$element is the Ollivier's Ricci curvature of node pair $(i,j)$,
\vspace{-0.03in}
\begin{equation}
[\boldsymbol R^\alpha(\boldsymbol A, \boldsymbol X)]_{ij}=1- \frac{ [\boldsymbol L^\alpha f(\boldsymbol X)]_i-[\boldsymbol L^\alpha  f(\boldsymbol X)]_j }{d(\boldsymbol x_i, \boldsymbol x_j)},
 \label{Ric}
 \vspace{-0.03in}
\end{equation}
with an affine transform $f: \mathbb R^{N \times F} \to \mathbb R^N$. 
Note that, \emph{our formulation of Ricci curvature in Eq. (\ref{Ric})  is differentiable with respect to the node features $\boldsymbol x$.}

Next, we prove that our formulation is a well approximation of Ollivier's Ricci curvature in Eq. (\ref{ORC}).
\newtheorem*{pro3}{Proposition 3 (Upper Bound)} 
\begin{pro3}
The differentiable Ricci curvature in Eq. (\ref{Ric}) is the upper bound of Ollivier's Ricci curvature in Eq. (\ref{ORC}),  $[\boldsymbol R(\boldsymbol A, \boldsymbol X)]_{ij}=\sup Ric^{\alpha}_{ij}$.
\end{pro3}
\vspace{-0.07in}
\begin{mymath}
\begin{proof}
Applying Kantorovich-Rubinstein duality \cite{DBLP:conf/nips/GulrajaniAADC17}, the Wasserstein distance between two distributions is rewritten as 
\begin{equation}
    W(p, q) = \sup \nolimits_{\lVert f \rVert_L \leq 1} \mathbb{E}_{z\sim p}[f(z)] - \mathbb{E}_{z\sim q}[f(z)], \label{krduality}
\end{equation}
where $f$ is $1-$Lipschitz.
With Eq. (\ref{pmf}), Eq. (\ref{alphaLaplacian}) and Eq. (\ref{krduality}), 
\begin{equation}
    \begin{aligned}
        W(m_u^\alpha, m_v^\alpha) 
        &= \sup \limits_{\lVert f \rVert_L \leq 1} \sum_{w \in \mathcal{V}} f(w)m_u^\alpha(w) - \sum_{w \in \mathcal{V}} f(w)m_v^\alpha(w) \\
        &= \sup \limits_{\lVert f \rVert_L \leq 1} [\boldsymbol L^\alpha f(\boldsymbol X)]_i-[\boldsymbol L^\alpha  f(\boldsymbol X)]_j, 
    \end{aligned}
    \label{sup}
\end{equation}
It is easy to verify that affine transform is $1-$Lipschitz with proper scaling according to Cauchy-Schwartz inequality.
Thus, $f $ is feasible for the supremum problem. With Eq. (\ref{Ric}), Eq. (\ref{ORC}) and Eq. (\ref{sup}), we have $[\boldsymbol R(\boldsymbol A, \boldsymbol X)]_{ij}=\sup Ric^{\alpha}_{ij}$ hold.
\end{proof}
\end{mymath}

%\noindent \textbf{Remarks.}
\vspace{-0.07in}
\noindent In particular, for the features $\boldsymbol X^m$ in the factor  $\mathbb G^{d_m}_{\kappa_m}$, the affine transform $f$ is parameterized as
\vspace{-0.05in}
\begin{equation}
f(\boldsymbol X^{\kappa_m})=\left(\boldsymbol W_m \otimes_{\kappa_m} \boldsymbol X^{\kappa_m}\right) \oplus_{\kappa_m} \boldsymbol b_m,
\vspace{-0.07in}
\end{equation}
where $\boldsymbol W_m$ and $\boldsymbol b_m$ denote the weight and bias. $\otimes_{\kappa_m}$ and $\oplus_{\kappa_m}$ are the gyrovector operations given in Appendix. Correspondingly, $f(\boldsymbol X)=\boldsymbol W_M \boldsymbol X+ \boldsymbol b_M$ for the Euclidean features.

% $f([\boldsymbol X^1: ...: \boldsymbol X^M])=\boldsymbol W^1 \otimes_{\kappa_1} \boldsymbol X^1 + \cdots + \boldsymbol W^M \otimes_{\kappa_M} \boldsymbol X^M + \boldsymbol b$,
% in latent Riemannian space thanks to the product construction,
% where $\otimes_{\kappa_1}$ is the gyrovector multiplication given in Appendix, and $\boldsymbol X^m$ are the features in the factor manifold.

\subsection{Structure Refinement with Ricci Flow}

In DeepRicci, we propose to refine graph structure in the latent Riemannian space in reminiscent of Ricci Flow.

%design a Ricci Flow generator to generate a refined graph structure with our differentiable Ricci curvature.

In differential geometry, 
Ricci flow \cite{Hopper2010} evolves a smooth manifold so that regions of large positive curvature tend to be more densely packed than regions of negative curvature, and finally the manifold divides itself into several submanifolds. 
In analogy to the smooth manifold, a graph trends to narrow the bottleneck so as to finally divide itself into several packed subgraphs in the Ricci flow. 
%and shrink the clusters in the Ricci flow.
% \emph{Intuitively, a graph generated backward the Ricci flow widens the bottlenecks on the original graph, and thus trends to relieve the over-squashing.}
% Our Ricci flow generator is designed according to this intuition that the optimized structure $\boldsymbol A^\star$ is generated backward the Ricci flow from the observed $\boldsymbol A$, widening the bottlenecks on $\boldsymbol A$. 
\emph{Intuitively, the previous state graph backward Ricci flow has ``wider'' bottleneck and thus alleviates over-squashing.}
We provide theoretical analysis in Sec. \ref{theory}, and  visualize the graph evolvement of Ricci flow in the Case Study.
% Our Ricci flow generator is designed according to this intuition that the optimized structure $\boldsymbol A^\star$ is generated backward the Ricci flow from the observed $\boldsymbol A$, widening the bottlenecks on $\boldsymbol A$. 

% \begin{equation}
% \begin{aligned}
%  d^{(t+1)}_{ij} & =(1-[\boldsymbol R^{(t)}(\boldsymbol A^\star, \boldsymbol X^\star)]_{ij})  d^{(t)}(\boldsymbol x^\star_i, \boldsymbol x^\star_j) \\
%  & = [\boldsymbol L^\alpha \boldsymbol f(\boldsymbol X^\star)]_i-[\boldsymbol L^\alpha \boldsymbol f(\boldsymbol X^\star)]_j 
%  \end{aligned}
% \end{equation}
Structure refinement in our proposal is based on the intuition above. 
Specifically, the Ricci flow on a graph \cite{Olli2010Survey} is given as,
\begin{equation}
\frac{\partial }{\partial t} d(\boldsymbol x_i, \boldsymbol x_j)=-Ric_{ij} d(\boldsymbol x_i, \boldsymbol x_j),
\label{RicciFlow}
\end{equation}
where $d(\boldsymbol x_i, \boldsymbol x_j)$ is the distance in the manifold, and we use the differentiable formulation of Ricci curvature $Ric_{ij}$. 
In our design, the observed structure $\boldsymbol A$ is  inferred from \emph{the previous state of optimized structure} $\boldsymbol A^\star$ backward Ricci flow.
%, and thus the distance in $\boldsymbol A$ is formulated according to Ricci flow as follows,
With Eqs.  (\ref{Ric}) and (\ref{RicciFlow}),  the distance in the observed graph is formulated,
\begin{equation}
\begin{aligned}
d(\boldsymbol x_i, \boldsymbol x_j) & =(1-[\boldsymbol R^{\alpha}(\boldsymbol A^\star, \boldsymbol X^\star)]_{ij})  d(\boldsymbol x^\star_i, \boldsymbol x^\star_j) \\
 & = [\boldsymbol L^\alpha(\boldsymbol A^\star) f(\boldsymbol X^\star)]_i-[\boldsymbol L^\alpha(\boldsymbol A^\star) f(\boldsymbol X^\star)]_j.
 \end{aligned}
 \label{backRicFlow}
\end{equation}
Note that, the distance in Eq. (\ref{backRicFlow}) is a function of  $\boldsymbol A^\star$ and $\boldsymbol X^\star$.
We learn the optimized structure $\boldsymbol A^\star$  by maximizing the likelihood of the observation as follows,
\begin{equation}
\mathcal L_{\operatorname{Struct}}=-\sum\nolimits_{i=1}^{N}\sum\nolimits_{j=1}^{N}\log p([\boldsymbol A]_{ij}=1| \boldsymbol A^\star).
\label{StructRefine}
\end{equation}
In particular, the likelihood is given by a Fermi-Dirac decoder \cite{DBLP:conf/nips/ChamiYRL19},
$ p([\boldsymbol A]_{ij}=1| \boldsymbol A^\star)=\operatorname{Sigmoid}\left(\frac{1}{s}\left( r-d(\boldsymbol x_i, \boldsymbol x_j)\right)\right)$, 
where $s$ and $r$ are parameters.

We consider the element in optimized structure as a random Bernoulli variable $[\boldsymbol A^\star]_{ij} \sim \operatorname{Ber}(\pi_{ij})$, parameterized by the pairwise similarity $\pi_{ij}$.
In latent Riemannian space, $\pi_{ij}$ takes the form of multihead cosine similarity as follows,
\begin{equation}
\pi_{ij}= \frac{1}{M}\sum\nolimits_{m=1}^{M}\cos\left(\boldsymbol S^m \phi^{\kappa_m}(\boldsymbol x^{\kappa_m}_i), \boldsymbol S^m \phi^{\kappa_m}(\boldsymbol x^{\kappa_m}_i) \right),
\end{equation}
where we have $M$ heads and $\boldsymbol S$ is the weight matrix. $\boldsymbol x^{\kappa_m}_i$ is the feature of Riemannian factor manifold, and $\phi^{\kappa_m}$  denotes the corresponding gyrovector  feature mapping. 
The issue is that $[\boldsymbol A^\star]_{ij}$ is not differentiable with respect to $\pi_{ij}$ in Bernoulli distribution.
Instead, we use the formulation below,
\begin{equation}
[\boldsymbol A^\star]_{ij}= \operatorname{Sigmoid}\left(\frac{1}{\tau}\left( \log \frac{\pi_{ij}}{1-\pi_{ij}}+\log \frac{\epsilon}{1-\epsilon}\right)\right),
\end{equation}
where $\epsilon$ is uniformly sampled from $(0,1)$ and $\tau \in \mathbb R^+$ for the Gumbel-sigmoid reparameterization \cite{DBLP:conf/sdm/Ng0FLC022}.
It gives the concrete relaxation of Bernoulli and, in this way, the binary $[\boldsymbol A^\star]_{ij}$ from a Bernoulli is transformed to a differentiable  function over $\epsilon$ and pairwise similarity $\pi_{ij}$.

\subsection{Feature Refinement with Geometric Contrastive Learning} \label{SecOfFeatureRefine}

In DeepRicci, we propose to simultaneously refine node feature by geometric contrastive learning, 
in which we consider the embedding generated from different Riemannian factors as different \textbf{geometric views}.
% in which node feature is concatenated with learnable parameters.

\emph{First, we model node features in the latent Riemannian space $\mathcal M$ with learnable parameters}.
Recall $\mathcal M=\mathcal P \otimes \mathcal F$, $\mathcal P = \otimes_{m=1}^{M-1} \mathbb G^{d_m}_{\kappa_m}$ where we utilize raw node feature $\boldsymbol x^{\operatorname{raw}}$ as the final factor $\mathcal F \in \mathbb R^F$ (Sec. \ref{TheSpace}).
For each node $v_i$, we have 
$\operatorname{Concat}(\boldsymbol x^{\kappa_1}, \cdots, \boldsymbol x^{\kappa_{M-1}}, \boldsymbol x^{\operatorname{raw}}) \in \mathcal M$, 
where $\boldsymbol x^{\kappa_m} \in \mathbb G^{d_m}_{\kappa_m}$ are learnable parameters, $m=1, \cdots, M-1$ and $M \ge 2$.

\emph{Second, we generate different geometric views from the product factors by a backbone GNN}.
The challenge here is that $\boldsymbol x^{\kappa_m}$ in the Riemannian factor cannot be fed into typical Euclidean GNNs.
Thanks to gyrovector  feature mapping  (Sec. \ref{LMap}), we map $\boldsymbol x^{\kappa_m}$ to Euclidean space, and generate  geometric view as follows,
\vspace{-0.05in}
\begin{equation}
\boldsymbol Z^{m} \gets \operatorname{GNN}\left(\boldsymbol A^\star, \phi^{\kappa_m}\left(\boldsymbol X^{\kappa_m}\right)| \Omega_{\operatorname{GNN}}\right),
\vspace{-0.05in}
\label{View}
\end{equation}
where $\Omega_{\operatorname{GNN}}$ is the parameter of backbone GNN, 
and $\boldsymbol A^\star$ is the optimized graph structure.
Node features in the factor manifold $\mathbb G^{d_m}_{\kappa_m}$ is summarized in $\boldsymbol X^{\kappa_m}$.
% and $\phi^{\kappa_m}$ denotes the corresponding gyrovector  feature mapping, which generates the geometric view $\boldsymbol Z^{m}$.
We utilize the gyrovector  feature mapping  $\phi^{\kappa_m}$, so that Euclidean GNN is able to generate the geometric view $\boldsymbol Z^{m}$.
In particular, we apply Fourier feature mapping  to generate the geometric view $\boldsymbol Z^{0}$.

%for raw features in Euclidean space

\emph{Third, we learn the refined feature by contrasting among different geometric views.}
Concretely, we contrast each geometric view generated from Rimannian factor and the geometric view from Euclidean features, and vice versa.
The contrastive loss is given by the popular InfoNCE \cite{DBLP:journals/corr/abs-1807-03748} as follows,
\vspace{-0.03in}
\begin{equation}
\operatorname{MI}(\boldsymbol Z^0, \boldsymbol Z^{m})=-\frac{1}{N}\sum^{N}_{i=1} \log \frac{\exp( Sim( \boldsymbol z_i^0, \boldsymbol z_i^{m} \rangle)}{\sum^{N}_{j=1}\exp( Sim(\boldsymbol z_i^0, \boldsymbol z_j^{m}) )},
\label{fRefine1}
\end{equation}
where $N$ is the number of nodes. $Sim(\boldsymbol x, \boldsymbol y)$ denotes the similarity measure in Euclidean space, and we use the standard inner product for simplicity.
Thus, we have the loss of feature refinement as follows, 
\vspace{-0.03in}
\begin{equation}
\mathcal L_{\operatorname{Feature}} =\frac{1}{M-1}\sum\nolimits_{m=1}^{M-1} \left( \operatorname{MI}(\boldsymbol Z^0, \boldsymbol Z^{m}) +\operatorname{MI}(\boldsymbol Z^{m}, \boldsymbol Z^0) \right),
\label{fRefine2}
\end{equation}
where $M$ is the number of geometric views.



% Recall that, the latent Riemannian space is designed as $\mathcal M=\mathcal P \otimes \mathcal F, \mathcal P = \otimes_{m=1}^{M-1} \mathbb G^{d_m}_{\kappa_m}$ 
% in which we utilize raw node feature $\boldsymbol x$ in $\mathbb R^F$ as the $M^{th}$ factor.
% We assign learnable parameters to each node $\{\boldsymbol x^{\kappa_m}\}_{m=1}^{M-1}$
% In this way, we obtain $M$ different geometric views o


%Instead of directly   an N-by-N $\boldsymbol A^\star$, 
% We generate optimized graph structure based on pairwise similarity, and similarity measure is parameterized a multi-head cosine as follows

\textbf{Overall Objective.} Incorporating Eq. (\ref{StructRefine}) and Eq. (\ref{fRefine2}) , the overall objective of self-supervised DeepRicci is formulated as 
\vspace{-0.1in}
\begin{equation}
\mathcal L_{\operatorname{DeepRicci}}=\beta \mathcal L_{\operatorname{Struct}}+(1-\beta) \mathcal L_{\operatorname{Feature}},
\vspace{-0.03in}
\end{equation}
where $\beta$ is a balancing factor between structure refinement and feature refinement.
\textbf{\emph{Finally, we accomplish structure-feature co-refinement with the novel latent Riemannian space in a self-supervised fashion,  alleviating the over-squashing.}}

\textbf{Complexity Analysis.} The overall process of training DeepRicci is summarized in Algorithm 1.
We construct the latent Riemannian space in Line $1$, and Line $2$ bridges it to Euclidean space.
We refine structure in Line $5-6$ and refine feature in Line $8-9$.
The parameters of GSL and GNN are jointly learnt in Line $11$.
The space complexity of the algorithm is $O(N^2)$ owing to the multihead cosine similarity in Line $6$, while $N$ is the number of nodes.
The time complexity is yielded as $O(N^2)$ owing to the geometric contrastive learning in Line $9$.
%The most expensive component is 7, yielding the complexity order of  and 
In other words, the complexity order of  DeepRicci is the same as that of the recent self-supervised GSL methods \cite{DBLP:conf/www/LiuZZCPP22,DBLP:conf/wsdm/0002WJZ023}, while we alleviate the over-squashing for boosting the performance of backbone GNN.

%We further detail the initialization step in the experiment.

% \begin{algorithm}[t] 
% \caption{\textbf{Self-supervised DeepRicci  }  } 
% \begin{algorithmic}[1] 
% \REQUIRE ~~\\ 
% Graph $G(\boldsymbol A, \boldsymbol X)$, A backbone GNN
% \ENSURE ~~\\ 
%  Optimized $G^\star(\boldsymbol A^\star, \boldsymbol X^\star)$, GNN parameters  $\Omega_{\operatorname{GNN}}$
%  \STATE Initialize feature augmentation $\boldsymbol x^{\kappa_m} \in \mathbb G^{d_m}_{\kappa_m}$;\
%  \WHILE{not converging}
% \STATE Perform feature map $\operatorname{LF}^\kappa_{a,b, \boldsymbol \omega}(\cdot)$ for $\boldsymbol x^{\kappa_m}, \forall m$;\\
%  \hfill $\rhd$ \emph{Structure Refinement}\\
% \STATE Compute differentiable Ricci curvatures in Eq. (\ref{Ric});\
% \STATE Refine structure $\boldsymbol A^\star$ with backward Ricci flow in Eq. (\ref{backRicFlow})-(\ref{StructRefine}); \\
% \hfill $\rhd$ \emph{Feature Refinement}\\
% \STATE Generate geometric views with GNN in Eq. (\ref{View});\
% \STATE Refine feature $\boldsymbol X^\star$ by contrasting among geometric  views in Eq. (\ref{fRefine1})-(\ref{fRefine2}). ;\\
% \hfill $\rhd$ \emph{Learn $G^\star$ and $\Omega_{\operatorname{GNN}}$}\\
% \STATE Compute gradient $\nabla_{ \{\boldsymbol x^{\kappa_m}\}_m, \Omega_{\operatorname{struct}}, \Omega_{\operatorname{GNN}} }\  \mathcal L_{\text{DeepRicci}}$;\
% \ENDWHILE
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
        \caption{     \textbf{Self-supervised DeepRicci  }      } 
        \KwIn{Graph $G(\boldsymbol A, \boldsymbol X)$, A Backbone GNN}
        \KwOut{Optimized $G^\star(\boldsymbol A^\star, \boldsymbol X^\star)$, Parameters  $\Omega_{\operatorname{GNN}}$
}
Initialize feature parameters $\boldsymbol x^{\kappa_m} \in \mathbb G^{d_m}_{\kappa_m}$;\\
\While{not converging}{   
        Perform feature map $\operatorname{GF}^\kappa_{\lambda,b, \boldsymbol \omega}(\cdot)$ for $\boldsymbol x^{\kappa_m}, \forall m$;\\
        \hfill $\rhd$ \emph{Structure Refinement}\\
        Compute differentiable Ricci curvature in Eq. (\ref{Ric});\\
        Refine structure with backward Ricci flow in Eqs. (\ref{backRicFlow})-(\ref{StructRefine}); \\
        \hfill $\rhd$ \emph{Feature Refinement}\\
        Generate geometric views with GNN in Eq. (\ref{View});\\
        Refine feature by contrasting among geometric  views in Eqs. (\ref{fRefine1})-(\ref{fRefine2}). ;\\
        \hfill $\rhd$ \emph{Jointly Learn $G^\star$ and $\Omega_{\operatorname{GNN}}$}\\
        Compute gradient $\nabla_{ \{\boldsymbol x^{\kappa_m}\}_m, \Omega_{\operatorname{GNN}} }\  \mathcal L_{\operatorname{DeepRicci}}$;\
}
\end{algorithm}



\begin{table*}
\vspace{-0.05in}
\caption{Node Classification on Cora, Citeseer, Chameleon and  Squirrel Datasets. (Best results: \textbf{Bold}, Runner up: \underline{\textit{Underlined}}.)}
\vspace{-0.05in}
\begin{tabular}{c  l | c c c | c c c | c c c | c c c }
\hline
& \multirow{2}{*}{\textbf{Method}  } & \multicolumn{3}{c|}{ \textbf{Cora}} & \multicolumn{3}{c|}{ \textbf{Citeseer}} & \multicolumn{3}{c|}{  \textbf{Chameleon}}& \multicolumn{3}{c}{  \textbf{Squirrel }} \\
&    & ACC & W-F1& M-F1  & ACC & W-F1& M-F1 & ACC & W-F1& M-F1 & ACC & W-F1& M-F1  \\
\hline
\multirow{9}{*}{\rotatebox{90}{    GCN } }   
& Original       
& 79.4\tiny{±0.4}  & 79.4\tiny{±0.4}  & 78.8\tiny{±0.3}  & 64.8\tiny{±0.6}  & 65.6\tiny{±0.6}  & 62.6\tiny{±0.6}  
& 32.2\tiny{±2.8}  & 30.5\tiny{±3.5}  & 30.5\tiny{±3.3}  & 22.2\tiny{±1.2}   & 21.9\tiny{±1.2}  & 21.9\tiny{±1.2} \\
& DropEdge         
& 80.4\tiny{±0.4}  & 80.8\tiny{±0.4}  & 79.4\tiny{±0.3}  & 67.6\tiny{±0.2}  & 68.3\tiny{±0.3}  & 65.0\tiny{±0.3}  
& 43.1\tiny{±0.5}  & 42.2\tiny{±0.8}  & 41.4\tiny{±0.9}  & 25.8\tiny{±1.2} & 25.1\tiny{±1.4} & 24.8\tiny{±1.5} \\
% & NeuralSparse   
% & 79.1\tiny{±1.3}&  79.1\tiny{±1.4}&  78.2\tiny{±1.4} & 68.7\tiny{±1.2}&  68.9\tiny{±1.2}& 66.9\tiny{±1.7}
% & 47.9\tiny{±2.6}&  44.9\tiny{±3.0}&  44.9\tiny{±2.8}  & 29.0\tiny{±1.1} & 28.1\tiny{±1.8} &  27.9\tiny{±1.9}  \\
& IDGL               
& 78.7\tiny{±0.6}  & 78.7\tiny{±0.9}  & 77.7\tiny{±0.9}  & 66.0\tiny{±0.8}  & 66.8\tiny{±0.8}  & 63.2\tiny{±0.9}  
& 42.2\tiny{±1.8}  & 40.8\tiny{±1.7}  & 39.8\tiny{±1.7}  & 25.8\tiny{±2.2} & 13.8\tiny{±2.3} & 13.6\tiny{±2.2} \\
& PRI-GSL            
& 79.3\tiny{±0.4}  & 79.3\tiny{±0.4}  & 78.8\tiny{±0.6}  & 67.1\tiny{±1.0}  & 67.9\tiny{±0.9}  & 64.0\tiny{±0.9}  
& \underline{\textit{51.8}}\tiny{±0.2}  & \underline{\textit{51.3}}\tiny{±0.4}  & \underline{\textit{51.0}}\tiny{±0.5}  & 28.7\tiny{±1.2} & 27.7\tiny{±2.1} & 27.4\tiny{±2.2} \\
& PASTEL           
& \underline{\textit{82.6}}\tiny{±0.5}  & \underline{\textit{82.5}}\tiny{±0.3}  & 81.2\tiny{±0.3}  & \underline{\textit{72.1}}\tiny{±1.1} & \underline{\textit{72.3}}\tiny{±0.8}  & \textbf{69.3}\tiny{±0.9}  
& \textbf{57.8}\tiny{±1.6}  & \textbf{57.8}\tiny{±2.4}  & \textbf{57.3}\tiny{±2.4}  & \textbf{37.5}\tiny{±0.2} & \textbf{37.5}\tiny{±0.6} & \textbf{37.5}\tiny{±0.7} \\
\cline{2-14}
& SLAPS            
& 79.8\tiny{±1.0}  & 80.1\tiny{±0.7}  & 79.3\tiny{±0.2}  & 65.7\tiny{±0.5}  & 66.2\tiny{±0.5} & 63.8\tiny{±0.1}  
& 33.9\tiny{±1.3}  & 34.1\tiny{±0.2}  & 31.5\tiny{±1.8}  & 23.2\tiny{±0.7}  & 22.7\tiny{±0.3} & 21.6\tiny{±0.3} \\
& SUBLIME           
& 82.3\tiny{±0.4}  & \underline{\textit{82.5}}\tiny{±0.4}  & \underline{\textit{81.5}}\tiny{±0.4}  & 71.0\tiny{±1.0}  & 71.4\tiny{±1.0}  & 67.6\tiny{±1.0}  
& 38.7\tiny{±1.4}  & 37.6\tiny{±1.3}  & 37.4\tiny{±1.3}  & 25.6\tiny{±0.4}  & 23.8\tiny{±2.2} & 23.9\tiny{±2.1} \\
& GSR               
& 80.9\tiny{±0.2}  & 81.1\tiny{±0.2}  & 80.2\tiny{±0.02} & 69.0\tiny{±0.3}  & 68.8\tiny{±0.3}  & 65.1\tiny{±0.3}  
& 43.6\tiny{±0.8}  & 42.8\tiny{±0.9}  & 42.1\tiny{±0.9}  & 25.8\tiny{±0.4} & 23.5\tiny{±0.5} & 23.7\tiny{±0.5} \\
& \textbf{DeepRicci}
& \textbf{82.8}\tiny{±0.6} & \textbf{82.7}\tiny{±0.6}  & \textbf{81.9}\tiny{±0.4}  & \textbf{72.3}\tiny{±0.8}  & \textbf{72.5}\tiny{±0.7} & \underline{\textit{68.6}}\tiny{±0.4}  
& 48.6\tiny{±0.8}  & 48.6\tiny{±0.8}  & 48.2\tiny{±0.8}  & \underline{\textit{28.9}}\tiny{±0.6} & \underline{\textit{28.4}}\tiny{±0.7} & \underline{\textit{28.1}}\tiny{±0.7} \\
\hline
\multirow{9}{*}{\rotatebox{90}{    GAT} }     
& Original
& 77.9\tiny{±0.6}  & 78.3\tiny{±0.6}  & 77.7\tiny{±0.5}  & 63.9\tiny{±2.5}  & 64.4\tiny{±1.7}  & 60.6\tiny{±1.7}  
& 32.0\tiny{±2.6}  & 29.9\tiny{±3.5}  & 29.9\tiny{±3.1}  & 22.6\tiny{±1.2} & 20.5\tiny{±1.4} & 20.5\tiny{±1.4} \\
& DropEdge           
& 78.4\tiny{±0.6}  & 78.7\tiny{±1.3}  & 76.9\tiny{±1.5}  & 65.9\tiny{±0.4}  & 66.2\tiny{±0.4}  & 62.8\tiny{±0.5}  
& 32.1\tiny{±2.6}  & 30.3\tiny{±1.6}  & 30.2\tiny{±1.2}  & 26.0\tiny{±1.0} & 25.6\tiny{±1.1} & 25.6\tiny{±1.0} \\
% & NeuralSparse      
% & 81.6\tiny{±4.2}&  81.4\tiny{±4.8}&  79.4\tiny{±4.8} & 65.1\tiny{±1.2}&  64.8\tiny{±1.5}& 61.9\tiny{±1.3}
% & 46.2\tiny{±2.0}&  45.6\tiny{±2.1}&  45.4\tiny{±1.8} & 30.2\tiny{±1.5} & 28.8\tiny{±1.3} &  28.8\tiny{±1.2} \\
& IDGL               
& 81.1\tiny{±1.0}  & 80.6\tiny{±1.0}  & 79.7\tiny{±0.9}  & 67.2\tiny{±1.3}  & 66.5\tiny{±1.5}  & 61.9\tiny{±1.8}  
& 49.1\tiny{±3.1}  & 48.4\tiny{±4.0}  & 47.8\tiny{±3.1}  & 29.5\tiny{±2.4} & 27.0\tiny{±2.6} & 27.0\tiny{±2.3} \\
& PRI-GSL            
& 79.7\tiny{±0.6}  & 79.7\tiny{±0.6}  & 78.5\tiny{±0.9}  & 66.1\tiny{±0.4}  & 66.2\tiny{±1.0}  & 62.6\tiny{±1.1}  
& 48.0\tiny{±2.4}  & 46.8\tiny{±2.3}  & 46.2\tiny{±2.4}  & 24.6\tiny{±0.9}  & 23.0\tiny{±2.1}  & 23.0\tiny{±2.9} \\
& PASTEL           
& 81.9\tiny{±1.4}  & \underline{\textit{81.9}}\tiny{±1.4}  & 80.7\tiny{±1.2}  & 66.8\tiny{±1.6} & 66.6\tiny{±1.9} & 62.0\tiny{±1.7}  
& \textbf{52.2}\tiny{±1.9}  & \textbf{52.1}\tiny{±2.7}  & \textbf{52.5}\tiny{±2.8}  & \underline{\textit{35.0}}\tiny{±1.1} & \underline{\textit{34.8}}\tiny{±1.3} & \underline{\textit{34.8}}\tiny{±1.3} \\
\cline{2-14}
& SLAPS            
& 78.2\tiny{±0.7}  & 78.3\tiny{±0.7}  & 77.3\tiny{±1.0}  & 64.8\tiny{±0.9} & 65.1\tiny{±1.2} & 61.7\tiny{±0.6}  
& 33.6\tiny{±1.8} &  29.5\tiny{±1.3}  & 28.4\tiny{±1.7}  & 19.0\tiny{±0.6} & 16.4\tiny{±0.3} & 15.8\tiny{±0.8}  \\
& SUBLIME            
&  \underline{\textit{82.2}}\tiny{±0.6} & 81.7\tiny{±0.7}  &  \underline{\textit{81.2}}\tiny{±0.6}   &  69.2\tiny{±1.2} &  \underline{\textit{69.7}}\tiny{±1.1}  &  \underline{\textit{66.0}}\tiny{±1.0}  
&  36.1\tiny{±0.6} &  35.6\tiny{±0.7}  &  35.6\tiny{±0.7}   &  24.7\tiny{±1.1} &  24.7\tiny{±1.1}  &  24.7\tiny{±1.1}  \\
& GSR               
& 81.8\tiny{±1.2}  & 81.8\tiny{±1.3}  & 80.9\tiny{±1.4}  & \underline{\textit{69.4}}\tiny{±1.0}  & 69.4\tiny{±0.9}  & 65.8\tiny{±0.9}  
& 37.8\tiny{±0.4}  & 36.0\tiny{±0.2}  & 35.7\tiny{±0.2}  & 26.7\tiny{±0.3} & 20.4\tiny{±0.1} & 20.5\tiny{±0.1} \\
& \textbf{DeepRicci}
& \textbf{82.2}\tiny{±0.5} &  \textbf{82.1}\tiny{±0.5}  & \textbf{81.6}\tiny{±0.2}  & \textbf{71.2}\tiny{±2.0} & \textbf{70.7}\tiny{±1.8} &  \textbf{68.9}\tiny{±0.5}       
& \underline{\textit{49.3}}\tiny{±1.3}  & \underline{\textit{49.1}}\tiny{±0.9}  & \underline{\textit{48.4}}\tiny{±1.1}  & \textbf{35.2}\tiny{±1.3} & \textbf{35.1}\tiny{±1.1} & \textbf{34.9}\tiny{±1.0} \\
\hline
\multirow{9}{*}{\rotatebox{90}{   SAGE} }
& Original                    
& 75.2\tiny{±1.3}  & 75.4\tiny{±1.6}  & 74.1\tiny{±1.6}  & 64.8\tiny{±1.8}  & 64.8\tiny{±1.6}  & 60.7\tiny{±1.6}  
& 39.9\tiny{±0.6}  & 39.2\tiny{±0.6}  & 39.5\tiny{±0.6}  & 27.6\tiny{±1.1} & 25.6\tiny{±1.5} & 25.6\tiny{±1.5} \\
& DropEdge          
& 79.9\tiny{±0.7}  & 80.5\tiny{±0.6}  & 79.1\tiny{±0.7}  & 66.7\tiny{±1.9}  & 67.7\tiny{±1.6}  & 63.9\tiny{±1.8}  
& 40.9\tiny{±1.1}  & 38.8\tiny{±1.0}  & 39.1\tiny{±0.9}  & 28.2\tiny{±1.0} & 26.1\tiny{±1.1} & 26.3\tiny{±1.0} \\
% & NeuralSparse      
% & 80.2\tiny{±1.8}&  79.7\tiny{±1.8}&  77.8\tiny{±1.6} &  65.3\tiny{±1.3}&  64.7\tiny{±1.4}& 61.1\tiny{±1.3}
% &  39.5\tiny{±1.9}&  39.1\tiny{±1.9}&  39.0\tiny{±1.8} & 33.7\tiny{±2.0} & 32.2\tiny{±2.4} &  32.2\tiny{±2.3} \\
& IDGL               
& 79.6\tiny{±0.8}  & 79.2\tiny{±0.9}  & 78.4\tiny{±0.8}  & 65.3\tiny{±1.1}  & 65.6\tiny{±0.9} & 61.3\tiny{±1.2}  
& 41.6\tiny{±2.1}  & 41.2\tiny{±2.0}  & 41.0\tiny{±1.3}  & 35.1\tiny{±0.9} & 33.9\tiny{±0.9} & 33.7\tiny{±0.8} \\
& PRI-GSL          
& 79.9\tiny{±0.5}  & 80.0\tiny{±0.5}  & 79.1\tiny{±0.4}  & 65.6\tiny{±0.9}  & 65.9\tiny{±0.9}  & 62.2\tiny{±0.8}  
& 39.8\tiny{±0.3}  & 35.2\tiny{±1.5}  & 34.3\tiny{±1.4}  & 19.3\tiny{±0.5}  & 14.2\tiny{±1.5}  & 14.9\tiny{±1.4}  \\
& PASTEL           
& 81.0\tiny{±0.8}  & 81.1\tiny{±0.8}  & 79.8\tiny{±0.7}  & 65.7\tiny{±1.0} & 65.9\tiny{±1.1}  & 61.4\tiny{±1.4}  
& \textbf{47.5}\tiny{±0.7}  & \textbf{47.7}\tiny{±0.9}  & \textbf{46.9}\tiny{±0.9}  & \underline{\textit{35.6}}\tiny{±1.2} & \underline{\textit{34.3}}\tiny{±1.5} & \underline{\textit{34.3}}\tiny{±1.5} \\
\cline{2-14}
& SLAPS      
&  77.4\tiny{±1.1}  &  76.3\tiny{±0.8}    &  76.2\tiny{±0.8}     &  65.1\tiny{±2.8}  &  64.8\tiny{±0.7}    &  61.0\tiny{±0.9}
&  36.1\tiny{±2.2}  &  31.8\tiny{±1.2}    &  32.2\tiny{±1.0}     &  20.6\tiny{±1.5}  &  17.8\tiny{±0.6}    &  17.2\tiny{±0.8} \\      
& SUBLIME           
&  \underline{\textit{82.8}}\tiny{±0.5}  &  \underline{\textit{82.9}}\tiny{±0.4}  &  \underline{\textit{81.7}}\tiny{±0.4}   & \underline{\textit{70.4}}\tiny{±0.5} & \underline{\textit{70.8}}\tiny{±0.8}  & \underline{\textit{66.2}}\tiny{±1.2}  
&  36.6\tiny{±0.4}  &  35.3\tiny{±0.5}  &  35.5\tiny{±0.5}   & 28.0\tiny{±2.1} & 20.0\tiny{±1.4} & 19.9\tiny{±1.5} \\
& GSR                
& 81.0\tiny{±0.05} & 81.2\tiny{±0.06} & 80.3\tiny{±0.02} & 68.8\tiny{±0.05} & 68.7\tiny{±0.04} & 65.0\tiny{±0.04} 
& 39.1\tiny{±0.05} & 36.3\tiny{±0.06} & 35.8\tiny{±0.06} & 23.7\tiny{±0.2} & 21.5\tiny{±0.3} & 21.7\tiny{±0.3} \\
& \textbf{DeepRicci} 
&  \textbf{83.2}\tiny{±0.3} &  \textbf{83.3}\tiny{±0.7} &  \textbf{82.9}\tiny{±0.6} &  \textbf{72.0}\tiny{±0.1} &  \textbf{72.2}\tiny{±0.4} & \textbf{69.1}\tiny{±0.5}
&  \underline{\textit{42.2}}\tiny{±0.7} &  \underline{\textit{41.9}}\tiny{±0.7} & \underline{\textit{41.8}}\tiny{±0.8}  &  \textbf{35.9}\tiny{±1.2} &  \textbf{35.7}\tiny{±1.0} & \textbf{35.7}\tiny{±1.2} \\
\hline   
    \end{tabular}
    \label{classification}
    \vspace{-0.1in}
    \end{table*}


\section{Theory on Over-squashing}\label{theory}

We further elaborate on the theoretical aspects of the proposed DeepRicci, and show \emph{the theoretical guarantee on alleviating over-squashing on the graph}. 

%We begin with a formal discussion on the phenomena of over-squashing.
Intuitively, useful information on the nodes is squashed when passing through the ``bottleneck'' on the graph, especially for the information from the long-distant nodes.
We employ the Cheeger's constant for  a formal discussion.
 \vspace{-0.03in}
\newtheorem*{def2}{Definition (Cheeger's Constant)} 
\begin{def2}
Given a $\mathcal G(\mathcal V, \mathcal E)$ with node set $\mathcal V$ and edge set $\mathcal E$, Cheeger's constant is defined as
 \vspace{-0.1in}
\begin{equation}
h_G= \min\nolimits_{\Omega \in \mathcal V}\frac{|\partial \Omega|}{\min\{vol(\Omega), vol(\bar{\Omega})\}},
 \vspace{-0.05in}
\end{equation}
where $\bar{\Omega}=\mathcal V \setminus \Omega$ is the complement of vertex set $\Omega$, and the boundary $\partial  \Omega=\{(x,y)\in\mathcal E: x\in \Omega, y\notin  \Omega \}$ is the set of all edges going from $\Omega$ to a node outside of $\Omega$.
\end{def2}
\noindent Cheeger's constant measures the degree of information squashing from nodes in $\Omega$ through its boundary, referred to as the ``bottleneck'' \cite{DBLP:conf/www/Liu0P00C023,DBLP:conf/iclr/ToppingGC0B22}. 
A smaller $h_G$ implies a narrowed bottleneck and severe over-squashing, while a larger $h_G$ alleviates over-squashing.
In fact, $h_G$ is controlled by the spectral gap.
\newtheorem*{lemma}{Lemma (Lower Bound \cite{Cheeger})} 
\begin{lemma}
The Cheeger's constant is lower bounded by $2h_G > \lambda_1$, where the spectral gap $\lambda_1$ is the first non-zero Laplacian eigenvalue of $G$.
\end{lemma}

In other words,  over-squashing is related to the spectral gap of the graph structure. We have the following proposition hold.
 %We will prove that our structure refinement in Eq. () increase the spectral gap.

%\subsection{Ricci Curvature \& Over-squashing}
%\cite{RicciCurvatureOfGraph}

\newtheorem*{pro4}{Proposition 4 (Over-squashing)} 
\begin{pro4}
The  refined structure  of DeepRicci alleviates over-squashing by increasing the Cheeger’s constant on the graph.
\end{pro4}

\begin{mymath}
\begin{proof}
According to \cite{Olli2010Survey}, the inequality $\lambda_1 > \kappa_0$ holds for any finite graph, where $\kappa_0$ is the minimum positive Ricci curvature on the edges. That is, $2h_G > \lambda_1 > \kappa_0$, and $\kappa_0$ is increased in backward Ricci flow, which is proved in \cite{Hopper2010}.
\end{proof}
\end{mymath}
\vspace{-0.05in}
\noindent An intuitive check is that the bottleneck is narrowed in forward Ricci flow, as will be shown in Sec. \ref{Case} (Case Study).

\vspace{-0.05in}
\section{Results \& Discussion}
\vspace{-0.05in}
% In this section, we compare the proposed DeepRicci with strong baselines on 4 public datasets with the aim of answering the research questions as follows (\emph{RQs}):
 In this section, we conduct extensive experiments to evaluate the proposed DeepRicci on $4$ public datasets with the aim of answering following research questions (\emph{RQs}):
\begin{itemize}
  % \item \emph{RQ1} (\textbf{Main Results}) How does the DeepRicci boost the downstream tasks?
  % \item \emph{RQ2} (\textbf{Ablation Study}) How does each component contributes to the success of DeepRicci?
  % \item \emph{RQ3} (\textbf{Case Study})  How does Ricci flow connected to relieving over-squashing?
    \item \emph{\textbf{RQ1}}. How does DeepRicci boost the downstream tasks?
  \item \emph{\textbf{RQ2}}. How does each module contribute to DeepRicci?
  \item \emph{\textbf{RQ3}}.  How does Ricci flow connect to over-squashing?
\end{itemize}

\vspace{-0.05in}
\subsection{Experimental Setup}
\vspace{-0.03in}

\subsubsection{Datasets \& Baselines}
We choose the public datasets of Cora, Citeseer, Chameleon and Squirrel \cite{sun23priGSL,DBLP:conf/cikm/SunLYFPJLY22}.
%whose statistics are given in Table \ref{statistics}.
\textbf{In this paper, we focus on the self-supervised GSL}.
Self-supervised baselines include the recent SUBLIME \cite{DBLP:conf/www/LiuZZCPP22}, and GSR  \cite{DBLP:conf/wsdm/0002WJZ023} of pretrain-finetune pipeline.
In addition, we include SLAPS  \cite{DBLP:conf/nips/FatemiAK21} which is trained by the denoising autoencoder only for self-supervised learning.
% Thus, we compare our model with recent self-supervised Sublime \cite{DBLP:conf/www/LiuZZCPP22}.
% GSR pretrains the graph and finetunes on node classification specifically \cite{DBLP:conf/wsdm/0002WJZ023}.
We also compare with \textbf{Supervised baselines}: 
DropEdge \cite{DBLP:conf/iclr/RongHXH20}, 
%NerualSparse \cite{DBLP:conf/icml/ZhengZCSNYC020}, 
IDGL \cite{DBLP:conf/nips/0022WZ20},
the recent PRI-GSL \cite{sun23priGSL}, 
and PASTEL \cite{DBLP:conf/cikm/SunLYFPJLY22}  addressing over-squashing in supervised manner.
We do not compare with the graph rewriting methods \cite{DBLP:conf/iclr/ToppingGC0B22,DBLP:conf/www/Liu0P00C023}, as they cannot jointly learn with GNNs and thus different from our propose.
We evaluate each method with the popular backbones of GCN \cite{DBLP:conf/iclr/KipfW17}, GAT \cite{DBLP:conf/iclr/VelickovicCCRLB18} and SAGE \cite{DBLP:conf/nips/HamiltonYL17}.
\emph{Existing GSL methods are Euclidean, and we for the first time introduce Riemannian geometry to GSL, to the best of our knowledge.}
%\subsubsection{Evaluation Metric}




% \begin{figure}
% \centering
%     \includegraphics[width=1\linewidth]{Ricci}
%      \caption{Case Study}
%     \label{CaseStudy}
% \end{figure}
\vspace{-0.05in}
\subsubsection{Reproducibility}
We introduce the implementation details  to enhance reproducibility.
For simplicity, we instantiate DeepRicci with $3-$factor rotational product $\mathcal M=\mathcal P \otimes \mathcal F$, 
where $\mathcal P$ is the product of a hyperbolic $\mathbb G^{32}_{-1}$ and a hyperspherical  $\mathbb G^{32}_{+1}$, enjoying the merit of different geometries.
The coefficient $\beta$ is set to $0.5$ by default, $\rho$ is a Gaussian distribution in practice.
The parameters $\boldsymbol x^\kappa$ of Riemannian manifolds are learned by Riemannian Adam \cite{DBLP:conf/iclr/BecigneulG19}, while the others are learned by standard Adam optimizer.
%where learning rate is $0.001$ and dropout is $0.3$ for both cases.
%Training DeepRicci typically takes $0.5$h for YYY datasets 
We conduct experiment on the server of  Intel Xeon Gold 5120T CPU and NVIDIA Tesla V100 GPU.
%and training our model on Cora typically takes $0.5$h. 
We initialize $\boldsymbol x^\kappa$ randomly in the gyrovector balls of $\mathbb G^{32}_{-1}$ and $\mathbb G^{32}_{+1}$ (Line 1 in Algorithm 1).
Alternatively, it can be initialized as the embeddings learned from any Riemannian GNN, e.g., \cite{DBLP:conf/icml/BachmannBG20}.
We conduct $5$ independent runs for each model, and report the mean and standard derivations.
\textbf{Codes} and further implementation details are given in \emph{https://github.com/RiemanGraph/}.


% \begin{table}
% \centering
% \vspace{-0.05in}
% \caption{Statistics of the datasets.}
% \vspace{-0.05in}
% \begin{tabular}{r  | c c  c c }
% \hline
% \textbf{Dataset} & Cora & Citeseer & Chameleon & Squirrel \\
% \hline
% \#(nodes)  &$2708$   &  $3327$&  $2277$  &  $5201$ \\
% \#(edges)  & $5429$ & $4732$ &  $36101$  & $217073$  \\
% \hline
% \end{tabular} 
% \label{statistics}
% \vspace{-0.25in}
% \end{table}

\vspace{-0.1in}
\subsection{Main Results}
\vspace{-0.03in}
We evaluate our model on node classification and clustering.

\subsubsection{Node Classification}
Three popular metrics are employed: classification accuracy (ACC), Weighted-F1 score (W-F1)  and Macro-F1 score (M-F1) (\%).
We summarize the results on all the $4$ datasets in Table \ref{classification}.
``Original'' denotes the results of backbone GNN without GSL.
The supervised GSL methods optimize structure learning and node classification jointly, while self-supervised methods are employed in the same manner as \cite{DBLP:conf/www/LiuZZCPP22} to ensure a fair comparison.
%is utilized same as Sublime  for fair comparison.
%and ours) obtain classification by a forward pass of the learnt backbone GNN.
In particular, GSR maintains its pretrain-finetune pipeline as described in the original paper \cite{DBLP:conf/wsdm/0002WJZ023}.
 \emph{\textbf{DeepRicci} consistently achieves the best results among self-supervised methods}, 
and even outperforms most supervised baselines, e.g., DeepRicci receives performance gain compared to the best supervised GSL on Cora.

\subsubsection{Node Clustering}
Three popular metrics are employed: clustering accuracy (ACC), Normalized Mutual Information (NMI) and Adjusted Rand Index (ARI) (\%).
Note that, the supervised GSL methods require node labels for learning an optimized graph, while clustering is unsupervised by nature.
Thus, supervised GSL methods cannot be applied to node clustering. 
In other words, only the self-supervised methods are suitable for node clustering, and we employ GCN as the backbone.
In particular, we utilize the pretrained embeddings of GSR \cite{DBLP:conf/wsdm/0002WJZ023} for clustering, as its finetune phase is designed for classification specifically.
%We apply K-Means to the node encodings, generated by the learnt backbone, and we use GCN backbone for clustering. 
We include K-Means as a reference, and also compare with a clustering method with the discrete Ricci curvature, RicciC \cite{RiccComm}.
In addition, we include recent \emph{Deep Graph Clustering} (DGC) methods:  CGC \cite{CGC}, gCooL\cite{gCooL}, HostPool \cite{HostPool} and AGC-DRR \cite{AGC-DRR}.
The results on Cora and Citeseer are reported in Table \ref{clustering}.
\emph{\textbf{DeepRicci} outperforms other GSL methods}, and consistently achieves the best results except NMI on Cora.
A reason is that the similarities in various geometric views of DeepRicci facilitate node clustering.
% in all the cases.


% &CGC   \citep{DBLP:journals/corr/abs-2204-08504}                     
% &   73.1 \tiny{(2.2)}    & 57.0 \tiny{(0.9)}    & 49.3 \tiny{(1.8)}     &   69.6 \tiny{(0.6)}     &  44.6 \tiny{(0.1)}   & 46.0 \tiny{(0.6)} 
% &gCooL  \citep{DBLP:conf/www/LiJT22}             
% &   72.0 \tiny{(1.6)}    & 58.3 \tiny{(0.2)}  & 56.9 \tiny{(0.9)}    & \underline{71.5} \tiny{(1.0)}    & 47.3 \tiny{(0.8)}    & 46.8 \tiny{(1.5)} 
% &HostPool  \citep{DBLP:conf/cikm/DuvalM22}            
% &   71.8 \tiny{(0.8)}  & 60.5 \tiny{(1.0)}  & \underline{58.5} \tiny{(1.1)}  & 70.9 \tiny{(0.5)}   & \underline{50.2} \tiny{(0.3)} &45.9 \tiny{(0.7)} 
% &AGC-DRR \citep{DBLP:conf/ijcai/GongZTL22}  
% &  40.6 \tiny{(0.6)}    & 18.7 \tiny{(0.7)}    & 14.8 \tiny{(1.6)}     &  68.3 \tiny{(1.8)}     & 43.3 \tiny{(1.4)}   & 45.3 \tiny{(2.3)} 
% &  RiccCom  \citep{CDRiccFlow} 
% &  55.6 \tiny{(0.3)}    & 58.1 \tiny{(1.1)}  & 48.9 \tiny{(0.9)}     &  67.3 \tiny{(1.2)}     & 46.2 \tiny{(0.8)}   & 44.9 \tiny{(0.6)} 


\begin{table}
\centering
\caption{Node Clustering (Best results: \textbf{Boldfaced}, Runner up: \underline{\textit{Underlined}}, Derivation is omitted for clarity.) }
\vspace{-0.05in}
\begin{tabular}{c l  | c c  c |c c c  }
\hline
&\multirow{2}{*}{\textbf{Method}  }  & \multicolumn{3}{c|}{ \textbf{Cora}} & \multicolumn{3}{c}{ \textbf{Citeseer}} \\
           &       & ACC & NMI & ARI  & ACC & NMI & ARI   \\
\hline
& K-Means &   $49.3$    & $32.5$    &$19.3$      & $54.4$      & $31.2$    &$28.5$   \\
\hline
\multirow{4}{*}{\rotatebox{90}{    DGC } } 
&CGC   & \underline{$\emph{72.7}$}& $56.1$    & $49.3$     &  $69.6$    &  $44.6$    & $45.0$  \\
&gCooL      &   $72.0$    & $55.3$    & $54.9 $     & \underline{$\emph{70.3}$}     & $45.8$  & \underline{$\emph{45.7}$} \\
&HostPool  &   $71.8$  & $\mathbf{60.2}$ &\underline{$\emph{55.3}$} & $70.1$  & \underline{$\emph{46.0}$}     & $45.2$  \\
&AGC-DRR&  $40.6$     & $19.3$   & $16.2 $     &  $68.3$    & $43.3$      & $44.1$ \\
\hline
& RicciC     &  $55.6$     & $54.8$    & $48.9 $      &  $67.3$    & $44.9$     & $44.2$ \\
\hline
\multirow{4}{*}{\rotatebox{90}{    GSL } } 
&SLAPS     &$ 69.2 $    & $54.9 $    &$37.4 $       & $67.1$    & $42.4$     & $39.2  $   \\
&Sublime   & $71.5$      & $54.1$    & $51.2$       &  $68.7$    & $44.3$     &  $43.9$  \\
&GSR         &$52.6 $      & $21.1$    & $24.0 $      & $59.2 $    & $29.5$     & $36.6 $   \\
&\textbf{DeepRicci}
 & $\mathbf{73.1}$ &\underline{$\emph{56.9}$}& $\mathbf{55.7}$ & $\mathbf{70.6}$  & $\mathbf{46.1}$ & $\mathbf{45.9}$ \\
\hline
\end{tabular} 
\vspace{-0.03in}
\label{clustering}
\end{table}


\begin{table}
\centering
\caption{Ablation Study on Classification.}
\vspace{-0.05in}
\begin{tabular}{c l | c c  c |c c c  }
\hline
& \multirow{2}{*}{\textbf{Variant}  } & \multicolumn{3}{c|}{ \textbf{Cora}} & \multicolumn{3}{c}{ \textbf{Citeseer}} \\
     &    & ACC & W-F1& M-F1  & ACC & W-F1& M-F1   \\
\hline
\multirow{4}{*}{\rotatebox{90}{GCN} } 
& \textbf{DeepRicci}
& $\mathbf{82.8}$ & $\mathbf{82.7}$ & $\mathbf{81.9}$ & $\mathbf{72.3}$  & $\mathbf{72.5}$ & $\mathbf{68.6}$  \\
& $-Gyro$  &$80.4 $&$81.0$ & $80.1$&$71.2$ & $72.0$&$ 67.9$  \\
& $-Ricci$   &\underline{$\emph{81.9}$} & \underline{$\emph{82.1}$} &\underline{$\emph{81.1}$} &$71.5$ &\underline{$\emph{72.2}$} & $68.3$  \\
& $-Feature$  &$80.8$ &$81.0$ & $80.3$ &\underline{$\emph{71.7}$} &$72.1$ & \underline{$\emph{68.6}$} \\
\hline
\multirow{4}{*}{\rotatebox{90}{SAGE} } 
& \textbf{DeepRicci}
    &  $\mathbf{83.2}$ &  $\mathbf{83.3}$ & $\mathbf{82.9}$ &  $\mathbf{72.0}$ & $\mathbf{72.2}$ &  $\mathbf{69.1}$ \\
& $-Gyro$ &$81.9 $ & $82.0 $& $ 80.3$&\underline{$\emph{70.1}$} & \underline{$\emph{70.4}$}&  \underline{$\emph{67.2}$} \\
& $-Ricci$     & \underline{$\emph{83.1}$} & $82.8 $& \underline{$\emph{82.6}$}&$69.3 $ & $69.7 $&  $66.6 $ \\
& $-Feature$ & $82.7 $ & \underline{$\emph{83.1}$}& $ 81.5$&$69.6 $ & $70.0 $&  $66.9 $ \\
\hline
\end{tabular} 
\label{ablation-classification}
\vspace{-0.2in}
\end{table}

\vspace{-0.07in}
\subsection{Ablation Study}
\vspace{-0.05in}
We examine the effectiveness of proposed components of DeepRicci: \emph{gyrovector  feature mapping}, \emph{backward Ricci flow} and \emph{feature refinement}.
%To this end, we introduce a variety of variants as follows.
To evaluate the gyrovector features, we introduce a variant (denoted as $-Gyro$) that replaces the gyrovector features $\phi^\kappa(\boldsymbol x^\kappa)$ with the logarithmic mapped features $\log^\kappa_{\boldsymbol 0}(\boldsymbol x^\kappa)$. 
The expression of $\log^\kappa_{\boldsymbol 0}(\cdot)$ is given in the Appendix.
The reference point of logarithmic map is the origin $\boldsymbol 0$, and note that  logarithmic map cannot take the point $\boldsymbol x^\kappa$ as the reference point \cite{DBLP:conf/icml/BachmannBG20}.
To evaluate Ricci flow, we introduce a variant (denoted as $-Ricci$) that disables the backward Ricci flow in structure refinement by setting $\beta=0$. 
To evaluate the significance of feature refinement, we introduce a variant (denoted as $-Feature$) that does not concatenate the gyrovector features $\phi^\kappa(\boldsymbol x^\kappa)$ for downstream tasks.
%Note that the parameter of $\boldsymbol x^\kappa$ is still required to construct the latent Riemannian space.
%That is, we feed the optimized structure $\boldsymbol A^\star$ and the raw feature into the backbone GNN.
We conduct ablation study on classification with the backbones of GCN and SAGE, and on clustering with GCN backbone.
The results on Cora and Citeseer are reported in Table \ref{ablation-classification} (classification) and Table \ref{ablation-clustering} (clustering), and we find that 
\textbf{(1)} The gyrovector features outperform the logarithmic features in all the cases.
Gyrovector features bridge Riemannian manifold and Euclidean space with an isometry-invariant kernel (\emph{Proposition 2}), while logarithmic map cannot generate Euclidean vectors with such guarantee.
\textbf{(2)} The model with backward Ricci flow achieves better results. We will further study on this point in the Case Study.
\textbf{(3)} Feature refinement generally boosts the performance of GNNs.
This is reasonable, as GNNs pass the message on the nodes, and noisy node feature trends to yield supoptimal embeddings for downstream tasks.
%node encodings generated by the GNNs are still based on the noisy node features.
\emph{It verifies the motivation of our study that refining the noisy features further boosts the performance of backbone GNN.}


\begin{table}[t]
\centering
\caption{Ablation Study on Clustering.}
\vspace{-0.05in}
\begin{tabular}{c l  | c c  c |c c c  }
\hline
&\multirow{2}{*}{\textbf{Variant}  }
                       & \multicolumn{3}{c|}{ \textbf{Cora}} & \multicolumn{3}{c}{ \textbf{Citeseer}} \\
 &                  & ACC & NMI & ARI  & ACC & NMI & ARI   \\
\hline
\multirow{4}{*}{\rotatebox{90}{    GCN } } 
& \textbf{\textbf{DeepRicci}}
                       & $\mathbf{73.1}$ & $\mathbf{56.9}$& $\mathbf{55.7}$ & $\mathbf{70.6}$  & $\mathbf{46.1}$ & $\mathbf{45.9}$ \\
& $-Gyro$& $70.9$  &  \underline{$\emph{55.2}$} &  $49.6$  &  \underline{$\emph{69.3}$} &  $43.9$  &  $44.7$  \\
& $-Ricci$  & \underline{$\emph{72.7}$} & $55.0$ &  \underline{$\emph{52.1}$}  &  $69.1$ &  \underline{$\emph{44.6}$}  &  \underline{$\emph{45.3}$}  \\
& $-Feature$ & $71.3$  &  $54.8 $ &  $49.2$  &  $68.7$ &  $44.2$  &  $45.1$  \\
\hline
\end{tabular} 
\label{ablation-clustering}
\end{table}

% \begin{figure}
% \vspace{-0.15in}
% \centering
%     \includegraphics[width=0.85\linewidth]{Ricci2}
%          \vspace{-0.1in}
%      \caption{Ricci Flow on Karate Club Network}
%     \label{CaseStudy}
% \vspace{-0.25in}
% \end{figure}

\begin{figure} 
 \vspace{-0.15in}
\centering 
\subfigure[Backward Ricci Flow]{
\includegraphics[width=0.75\linewidth]{1-cut}  \vspace{-0.2in}}
\subfigure[Forward Ricci Flow]{
\includegraphics[width=0.75\linewidth]{2-cut}  \vspace{-0.1in}}
 \vspace{-0.1in}
\caption{Visualization of Karate Club Network.}
 \vspace{-0.25in}
\label{CaseStudy}
\end{figure}

\vspace{-0.1in}
\subsection{Case Study: Ricci Flow \& Over-squashing} \label{Case}
\vspace{-0.05in}
Here, we empirically study the connection between Ricci flow and over-squashing.
To this end, we conduct case study on Karate Club network, visualized in Fig. \ref{CaseStudy}.
The backward subfigure is graph structure learnt by DeepRicci, while the forward subfigure is generated by another variant model where backward Ricci flow is replaced by a forward one.
Karate Club network has two communities, distinguished by the different colors in Fig. \ref{CaseStudy}.
% Forward Ricci flow divides the network into $3$ over-packed components, and components are not aligned with the groundtruth communities.
% It gives a extreme case that the information in each component cannot pass to each other as the ``bottleneck'' is broken.
The network evolves itself through forward Ricci flow to a state where two communities link to each other by a few edges. 
Consequently, information in the community is squashed when passing through such a narrow bottleneck.
\emph{Under backward Ricci flow, the bottleneck is ``widened'' by more linkages, motivating our design for structure refinement.}
Indeed, we further prove that backward Ricci flow alleviates over-squashing in Sec. \ref{theory}.


\vspace{-0.07in}
\section{Related Work}
\vspace{-0.05in}
\subsection{Graph Structure Learning}
\vspace{-0.05in}
In the literature, learning graph structure has been studied in traditional machine learning, e.g., spectral clustering and graph signal processing \cite{DBLP:conf/wsdm/WangZF22}.
In this paper, we focus on the Graph Structure Learning (GSL) \emph{for boosting GNNs with an optimized graph}.
%Given the graphs are usually noisy, graph structure learning aims to learn an optimized graph for GNNs.
%Existing GSL methods are roughly fallen into 2 categories. 
One line of work is driven by pairwise similarity.
The similarity is either measured by a kernel \cite{DBLP:conf/nips/0022WZ20}, 
or parameterized with a neural model \cite{sun23priGSL}.
\cite{DBLP:conf/nips/FatemiAK21} further improves GSL with a denoising autoencoder.
Gumble reparameterization trick is frequently used for optimizing the discrete graph structure \cite{DBLP:conf/nips/WuZLWY22}. 
Another line of work directly parameterizes the adjacency matrix, 
and training methods include bilevel optimization \cite{DBLP:conf/ijcai/HuCMS22}, 
%proximal gradient descent \cite{DBLP:conf/kdd/Jin0LTWT20,DBLP:conf/cikm/0011XYCW21}, 
%proximal gradient descent \cite{DBLP:conf/kdd/Jin0LTWT20}, 
Bayesian approach \cite{DBLP:conf/www/WangM0XJS021},
and variational inference \cite{DBLP:conf/kdd/SongZK22}.
Recent studies \cite{DBLP:conf/www/LiuZZCPP22,DBLP:conf/www/LiuWWC0S22,DBLP:conf/wsdm/0002WJZ023} incorporate contrastive learning  in GSL.
\cite{DBLP:conf/icml/LiuCSJ22} introduces an edge-to-vertex transform and its inverse.
\cite{DBLP:conf/www/ZouPHYLWLY23} conducts GSL by structural entropy.
\cite{DBLP:conf/icml/XieXJ22} infers a latent graph for self-supervised representation learning.
In addition, researchers study GSL on bipartite graphs \cite{DBLP:conf/nips/WeiLLW22}, 
%heterophily graphs \cite{DBLP:journals/corr/abs-2105-13795}, 
heterogeneous graphs \cite{DBLP:conf/aaai/ZhaoWSHSY21}, 
hypergraphs \cite{DBLP:conf/ijcai/CaiSSZH022}, etc.
We specify that the recent \cite{DBLP:conf/cikm/SunLYFPJLY22} alleviates over-squashing in Euclidean space, and is supervised by node labels.
%, but we consider the self-supervised scenario.
%As the node features are usually noisy as well, 
To the best of our knowledge, we for the first time address the self-supervised graph structure-feature co-refinement, alleviating over-squashing with theoretical guarantees.
%Also, it is noteworthy to mention that graph sparsification is a different problem that focus on ...

\vspace{-0.07in}
\subsection{Riemannian Geometry \& Graphs}
\vspace{-0.03in}
%Euclidean space has been the workhorse for studying graphs in the past decades. 
%It is not until recently that 
Riemannian geometry has emerged as a powerful tool to model graphs.
Among the Riemannian spaces, hyperbolic space is well aligned with the graphs with hierarchical or tree-like structures \cite{DBLP:conf/nips/LiuNK19,DBLP:conf/icml/00010Y0K23}, 
and hyperbolic GCNs of different formulations are introduced \cite{DBLP:conf/nips/ChamiYRL19,DBLP:conf/cvpr/DaiWGJ21}. 
$\kappa$-GCN \cite{DBLP:conf/icml/BachmannBG20} extends GCN to  constant curvature manifolds.
In ultrahyperbolic or quotient spaces,  \cite{DBLP:conf/nips/XiongZPP0S22,DBLP:conf/nips/Law21} study node embedding in the time-space coordinates of some curvature radius.
\cite{DBLP:conf/icml/LopezPT0W21} explores the symmetric matrix manifold for graphs.
\cite{DBLP:conf/nips/ZhuP00C020,DBLP:conf/www/YangCPLYX22} represent graphs with the dual spaces of Euclidean and hyperbolic ones.
\cite{sun21aaai} considers graph dynamics in hyperbolic space, while \cite{sun23aaai,sun22cikm} model graph sequences in Riemannian manifolds.
\cite{sun23jmlc} studies bipartite graph in evolving  manifolds.
 \cite{DBLP:conf/iclr/GuSGR19,sun22aaai}  study graph representation learning in the product space.
However, they do not model Ricci curvatures with the product space for structure learning.
Also, we notice that Ricci curvature is recently introduced for graph clustering \cite{sun23ijcai}, graph rewriting \cite{DBLP:conf/iclr/ToppingGC0B22} and edge dropping \cite{DBLP:conf/www/Liu0P00C023}, 
 but none of them learn a graph structure in absence of a differentiable Ricci curvature formulation.
Distinguishing from the existing studies, we introduce a latent Riemannian space with gyrovector map for GSL.

% On \emph{product manifolds}, \citet{GuSGR19,DBLP:conf/www/WangWSWNAXYC21,skopek2020mixed-curvature,sun2022self} explore informative embeddings in the collaboration of different factor manifolds.
% Additionally, \citet{DBLP:conf/aaai/CruceruBG21} study the matrix manifold of Riemannian spaces.
% Another line of work consider both Riemannian manifold and the Euclidean one.
% For example, \citet{zhu2020graph,DBLP:conf/www/YangCPLYX22} embed the graph into the dual space of Euclidean and hyperbolic ones simultaneously. 
% Recently, \citet{HTGN,DBLP:conf/cikm/0008YPY22} model the temporal network in hyperbolic manifolds.
% To the best of our knowledge, we introduce \emph{the first} co-evolving Riemannian manifolds, aligning with the characteristic of SINs.

\vspace{-0.1in}
\section{Conclusion}
\vspace{-0.05in}
In this paper, we pose a new problem of self-supervised graph structure-feature co-refinement, 
and propose \textbf{DeepRicci} from a fundamentally different perspective of Riemannian geometry, 
alleviating over-squashing with theoretical guarantees.
Specifically, we introduce a novel latent Riemannian space with gyrovector  feature mapping, 
where we refine structure by backward Ricci flow with differentiable Ricci curvature, and simultaneously refine feature by geometric contrastive learning among different Riemannian factors.
Extensive experiments on public datasets show the superiority of  DeepRicci.

\vspace{-0.05in}
% \section*{Appendix}
% \vspace{-0.03in}
% Gyrovector operations \cite{DBLP:conf/icml/BachmannBG20} utilized in this paper (i.e., M\"{o}bius addition $\oplus_\kappa$, gyrovector multiplication $\otimes_\kappa$ and  logarithmic map $\log_{\boldsymbol x}^\kappa$) are given as follows.
% \vspace{-0.05in}
% \begin{equation}
% \boldsymbol x \oplus_\kappa \boldsymbol y= \frac{(1-2\kappa\langle \boldsymbol x, \boldsymbol y\rangle+\kappa |\boldsymbol y|^2) \boldsymbol x+(1+\kappa |\boldsymbol x|^2) \boldsymbol y }{1-2\kappa\langle \boldsymbol x, \boldsymbol y\rangle+\kappa^2|\boldsymbol x|^2|\boldsymbol y|^2},
% \end{equation}
% \begin{equation}
% \vspace{-0.05in}
% \resizebox{0.89\hsize}{!}{$
%     \boldsymbol{M} \otimes_{\kappa} \boldsymbol{x} =\frac{1 }{ \sqrt{|\kappa|}} \tan_\kappa \left(\frac{|\boldsymbol{M} \boldsymbol{x}|}{|\boldsymbol{x}|} \tan_\kappa ^{-1}(\sqrt{|\kappa|}|\boldsymbol{x}|)\right) \frac{\boldsymbol{M} \boldsymbol{x}}{|\boldsymbol{M} \boldsymbol{x}|}, \label{mobius matrix multiplication}
% $}
% \end{equation}
% \begin{equation}
%     \log _{\boldsymbol{x}}^{\kappa}(\boldsymbol{y}) =\frac{2}{\lambda_{\boldsymbol{x}}^{\kappa}\sqrt{|\kappa|}} \tan _{\kappa}^{-1} |-\boldsymbol{x} \oplus_{\kappa} \boldsymbol{y}| \frac{-\boldsymbol{x} \oplus_{\kappa} \boldsymbol{y}}{ |-\boldsymbol{x} \oplus_{k} \boldsymbol{y} |. }, \label{log map}
%     \vspace{-0.07in}
% \end{equation}
% where $\lambda_{\boldsymbol{x}}^{\kappa}=\frac{2}{1+\kappa|\boldsymbol{x}|^{2}}$ is the conformal factor, and the curvature trigonometric function is defined as $\tan_{\kappa}(\cdot)=\tanh(\cdot)$ for $\kappa <0$, otherwise, $\tan_{\kappa}(\cdot)=\tan(\cdot)$.
% %\vspace{-0.03in}

